Geometric models of soliton vortex dynamics

We focus on BPS solutions of the gauged O(3) Sigma model, due to Schroers, and use these ideas to study the geometry of the moduli space. The model has an asymmetry parameter $\tau$ breaking the symmetry of vortices and antivortices on the field equations. It is shown that the moduli space is incomplete both on the Euclidean plane and on a compact surface. On the Euclidean plane, the L2 metric on the moduli space is approximated for well separated cores and results consistent with similar approximations for the Ginzburg-Landau functional are found. The scattering angle of approaching vortex-antivortex pairs of different effective mass is computed numerically and is shown to be different from the well known scattering of approaching Ginzburg-Landau vortices. The volume of the moduli space for general $\tau$ is computed for the case of the round sphere and flat tori. The model on a compact surface is deformed introducing a neutral field and a Chern-Simons term. A lower bound for the Chern-Simons constant $\kappa$ such that the extended model admits a solution is shown to exist, and if the total number of vortices and antivortices are different, the existence of an upper bound is also shown. Existence of multiple solutions to the governing elliptic problem is established on a compact surface as well as the existence of two limiting behaviours as $\kappa \to 0$. A localization formula for the deformation is found for both Ginzburg-Landau and the O(3) Sigma model vortices and it is shown that it can be extended to the coalescense set. This rules out the possibility that this is Kim-Lee's term in the case of Ginzburg-Landau vortices, moreover, the deformation term is compared on the plane with the Ricci form of the surface and it is shown they are different, hence also discarding that this is the term proposed by Collie-Tong to model vortex dynamics with Chern-Simons interaction.

==> chapters/cs-term/abelian-deformations/commands.tex <==

\newcommand*\vb[1]{\mathbf{ #1 }}


\DeclareDocumentCommand\brk{d()}{
  \left( #1 \right)
}

\newcommand*\surface{\Sigma}%

\DeclareMathOperator\potentialE{V}%

\newcommand*\nf{N}
\newcommand*\np{n}
\newcommand*\hf{\phi}%
\newcommand*\gp{a}%
\newcommand*\del{\partial}%
\newcommand*\sphere{{\mathbb{S}^2}}%
\newcommand*\Diff{\mathcal{D}}%
\newcommand*\conj[1]{\overline{#1}}%
\newcommand*\half{\frac{1}{2}}%
\newcommand*\pbundle{P}%
\newcommand*\fbundle{F}%
\newcommand*\north{n}%
\newcommand*\pconnection{A}%
\newcommand*\pcurvature{F}%
\newcommand*\isometry{\mathcal{I}}
%\newcommand*\abs[1]{\lvert{#1}\rvert}%

\NewDocumentCommand\abs{sm}{
  \IfBooleanTF#1{
    \left\lvert{#2}\right\rvert
  }{
    \lvert{#2}\rvert
  }
}

% \NewDocumentCommand\set{sm}{
%   \IfBooleanTF#1{
%     \left\{ #2 \right\}
%   }{
%     \{ #2 \}
%   }
% }


\newcommand*\laplacian{\Delta}%

\newcommand*\vset{\mathcal{P}}%

\newcommand*\avset{\mathcal{Q}}%

\newcommand*\moduli{\mathcal{M}}%
\newcommand*\modulikk{{\moduli^{k_+,k_-}}}

\newcommand*\eval[2]{\left.{#1}\right\rvert _{#2}}%

\newcommand*\cf{\Omega}
\newcommand*\reals{\mathbb{R}}%
\newcommand*\cpx{\mathbb{C}}%
\newcommand*\pSpace{\mathbb{P}}%

\DeclareMathOperator\Jop{J}%

\DeclareMathOperator\Vol{Vol}%

\DeclareMathOperator\Energy{E}

\newcommand*\order{\mathcal{O}}%

\newcommand*\ldv{\mathcal{L}}%
\newcommand*{\moduliMetric}{g}
\newcommand*{\dv}[1]{\frac{d}{d{#1}}}

\newcommand*\Lp[2][2]{\mathrm{L}^{#1}(#2)}

\DeclareDocumentCommand{\pdv}{m g}
{
  \IfValueTF{#2}
  {
    \frac{\del #1}{\del #2}
  }
  {
    \frac{\del }{\del #1}	
  }
}


%%%% Analysis
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}

\newcommand*\dd{d}
\newcommand*\length{\ell}
\newcommand*{\disk}{\mathbb{D}}
\newcommand*{\htilde}{\tilde{h}}
\newcommand*{\hstar}{h^*}
\newcommand*{\ctilde}{\tilde{c}}
\newcommand*\cstar{c^*}
\newcommand*{\hhat}{\hat{h}}
\newcommand*{\plane}{\R^2}
\newcommand*{\Fstable}{\mathcal{F}}
\newcommand*{\feps}{f_\epsilon}
\newcommand*\Csp[2][0]{\mathrm{C}^{#1}(#2)}
\newcommand*{\Hsp}{\mathrm{H}}
\newcommand*\Wsp{\mathrm{W}}
\newcommand*{\Lsp}{\mathrm{L}}
\newcommand*{\Xsp}{\mathcal{X}}
\newcommand*\Top{\mathrm{T}}
\newcommand*\Lop{\mathrm{L}}
%\newcommand*\norm[1]{\lvert\lvert#1\rvert\rvert}

\newcommand\dist{\mathrm{dist}}


\NewDocumentCommand\norm{sm}{
  \IfBooleanTF#1{
    \left\lvert\left\lvert#2\right\rvert\right\rvert
  }{
    \lvert\lvert#2\rvert\rvert
  }
}

\NewDocumentCommand\lproduct{sm}{
  \IfBooleanTF{#1}
  {\left\langle #2 \right\rangle}
  {\langle #2 \rangle}
}

\newcommand*{\Hnorm}[3][1]{\norm{#2}_{\Hsp[#1]{#3}}}
\newcommand*{\Lnorm}[3][2]{\norm{#2}_{\Lsp[#1]{#3}}}
\newcommand*{\Lprod}[2][\sphere]{\langle #2 \rangle_{#1}}

\newcommand*{\set}[1]{\left\{#1\right\}}

\newcommand*{\vd}[1]{
  \IfEqCase{#1}{
    {1}{v'}
    {2}{v''}
  }[\PackageError{V}{Only 1 or 2 allowed as options, got #1}{}]
}

\newcommand*\uniformlyto\rightrightarrows
\newcommand*\htildeEps{\htilde^\epsilon}
\newcommand*\ctildeEps{\ctilde^\epsilon}
\newcommand*\vdeps[1]{{\vd{#1}}^\epsilon}
\newcommand*\grad{\nabla}
\newcommand*\delEps{\del_\epsilon}
\newcommand*\proj{\mathbb{P}}


%Linear section commands
\newcommand*\ueps{u}
\newcommand*\afn{a}
\newcommand*\bfn{b}
\newcommand*\manifold{M}
\newcommand*\metric[1]{\langle{#1}\rangle}
\newcommand*\aForm{\mathcal{A}}
% \newcommand*\fFunc{\mathcal{F}}
\newcommand*\fFunc{B}
\newcommand*\hSp{\mathcal{H}}
\newcommand*\uBound{K_1}
\newcommand*\cBound{K_2}
\newcommand*\vol{\mathrm{Vol}}
\newcommand*\suchthat{\;\middle\vert\;}
\newcommand*\intManifold{\int_{\manifold}}
\newcommand*\vortexSet{\mathcal{P}}
\newcommand*\avortexSet{\mathcal{Q}}
\newcommand*\vavSet{\mathcal{S}}
\newcommand*\Dfrechet{\mathcal{D}}

%%%%%%%%%%%

\newcommand*\brackets{}

%%%%%%%%%%%

% Spaces

\newcommand*\domain{\mathscr{D}}
\newcommand\SobSp{W}

%\DeclareMathOperator\Lsp{L}
%\DeclareMathOperator\Hsp{H}

%\newcommand*\lsp[1]{\Lsp^{#1}}
%\newcommand*\hsp[1]{\Hsp^{#1}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "mhcs-param-notes.tex"
%%% End:


==> chapters/cs-term/abelian-deformations/sections/bounds-var.tex <==
%%%% LOCAL LaTeX %%%%%%%%%%%%%%%%%%
\newcommand*\ux{\underline x}
\newcommand*\ox{\overline x}

\newcommand*\Ik{I_{\kappa}}
\newcommand*\Aset{\mathcal{A}}
\newcommand*\avh{\overline{h}}
\newcommand*\Kset{\mathcal{K}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{The unbalanced case}

We prove some necessary conditions for the solution of the elliptic
problem to exist. In this section we assume $k_+ \neq k_-$. Let $N' =
\kappa N$, equation~~\eqref{eq:N} can be rewritten as, 
%
\begin{equation}
  \label{eq:N'}
  \laplacian N' + (\kappa^2 + 2F'(v + h))\,N' + \kappa^2F(v + h) = 0.
\end{equation}

Let $\ux = \min_{\surface} \set{N'(x)}$, $\ox = \max_{\surface}\set{
  N' }$, if we denote by $F(x) = F(v(x) + h(x))$ and $F'(x) = F'(v(x)
+ h(x))$, by the maximum principle,
%
\begin{align*}
-\frac{\kappa^2F(\ux)}{\kappa^2 + 2F'(\ux)} \leq
N'(x) \leq
- \frac{\kappa^2 F(\ox)}{\kappa^2 + 2F'(\ox)}.
\end{align*}

Since $F'(x) \geq 0$, we conclude the uniform bounds,
%
\begin{align}\label{eq:N'-bound}
-(1 + \tau) \leq N' \leq (1 - \tau).
\end{align}

From equations \eqref{eq:h}  and \eqref{eq:N'} we obtain,
%
\begin{align*}
\laplacian N'- \frac{\kappa^2}{2} \brk(\laplacian h + \frac{4\pi}{\abs
\surface} (k_+ - k_-)) + 2F'(v + h)N' = 0. 
\end{align*}

Integrating this equation,
%
\begin{align*}
-2\pi\kappa^2(k_+ - k_-) + 2 \lproduct{F'(v + h), N'} = 0.
\end{align*}

Using the fact that $F'$ is a positive function bounded by
$1/2$ and the uniform bound for $N'$,
%
\begin{equation*}
\kappa^2 = \frac{\lproduct{F'(v + h), N'}}{\pi(k_+ - k_-)}
  \leq \frac{\max\set{1 \mp \tau} \abs\surface}{2\pi\abs{k_+ - k_-}}.
\end{equation*}

Therefore, the family of deformation constants is bounded, contrasting with the
ecuclidean case, in which there are cases for which the elliptic
problem can be solved for any $\kappa$ \cite{chen2019analysis}. We
will denote by $C$ a positive constant 
that can change from one equation to the other, from \eqref{eq:N'} we
have a uniform bound for the norm of $N'$ in Sobolev's space, 
%
\begin{equation*}
  \norm{\laplacian N'}_{0,p} \leq C(p), \qquad p \geq 2.
\end{equation*}

By Calderon-Sygmund theory, this implies,
%
\begin{equation*}
  \norm{N'}_{2,p} \leq C \brk(
  \norm{\laplacian N'}_{0,p} + \norm{N'}_{0,p}
  ) \leq C.
\end{equation*}

If we fix any $p > 2$, Sobolev's theory says that the embedding
$\Wsp(2, p) \to C^1(\surface)$ is continuous, then there 
exist constants independent of $\kappa$, such that,
%
\begin{equation*}
  \norm{N'}_{C^1} \leq C_1\norm{N'}_{2, p} \leq C_2.
\end{equation*}

Similarly, if $\avh = \lproduct{h, 1}/\abs\surface$ is
the average of a solution $h$ to \eqref{eq:h}, then the set
$\set{h_{\kappa} - \avh_{\kappa}}$, where $h_{\kappa}$ is a solution for any given
parameter $\kappa$, is also uniformly bounded in $C^1$. 

\subsection{Limit points of solutions as $\kappa \to 0$}

Let $(h_n, N'_n)$ denote a sequence of solutions to the
elliptic equations \eqref{eq:h}-\eqref{eq:N'} with a corresponding
sequence of parameters $\set{\kappa_n}$. We are interested in
describing the behaviour of these solutions as $\kappa_n \to 0$. We can
not rule out the possibility that $\avh_n \to \pm \infty$,
therefore, we assume firstly that $h_n - \avh_n \to
\tilde h$ and $N'_n \to N'_0$ in $\Hsp^1$ as $\kappa_n \to 0$. We
distinguish two cases. First, if $\avh_n \to c$ for some real number
$c$, then $h_n \to h_0$ in $\Hsp^1$, where $h_0 = \tilde h + c$. In
this case, $(h_0, N'_0)$ is a weak solution of \eqref{eq:h},
\eqref{eq:N'} with $\kappa = 0$, by elliptic theory, they are also a
classical solution of the equations, but we know that for $\kappa = 0$
the equations describe the vortex-antivortex situation in which case 
uniqueness implies that $N'_0 \equiv 0$ and $h_0$ is the only solution of
the regularised vortex-antivortex equation,
%
\begin{equation*}
  \laplacian h_0 + 2 F(v + h_0) + \frac{4\pi}{\abs\surface} (k_+ -
  k_-) = 0.
\end{equation*}

For the second case, let us assume $\avh_n \to \pm \infty$, from
equation \eqref{eq:h},
%
\begin{equation*}
  \bar N'_n \abs\surface + \lproduct{F(v + h_n), 1} + 2\pi(k_+ - k_-)
  = 0.
\end{equation*}

Since $N'_n \to N'_0$ in $\Lsp^2$, we have the convergence $\bar N'_n
\to \bar N'_0$ and since $h_n - \avh_n$ is uniformly bounded, by the
dominated convergence theorem,
%
\begin{equation*}
 \lproduct{F(v + h_n), 1} \to (\pm 1 + \tau)\abs\surface.
\end{equation*}

Hence, $\bar N'_0 = \mp 1 - \tau - \frac{2\pi (k_+ -
  k_-)}{\abs\surface}$. Since $F(v + h_n)$ is bounded for any $h_n$,
 $F'(v + h_n) \to 0$ pointwise and $N'_n$ is uniformly bounded, we
 deduce by \eqref{eq:N'}  and the dominated convergence theorem, that
 $\norm{\laplacian N'_n}_{0, p} \to 0$ for any $p > 2$. Therefore, by
 Schauder's estimates and Sobolev's embedding, we deduce that,
 %
 \begin{equation*}
   \norm*{N'_n - \brk(\mp 1 - \tau - \frac{2\pi(k_+ -
       k_-)}{\abs\surface})}_{C^1} \to 0.
 \end{equation*}

 Now, from \eqref{eq:h} we have,
 %
 \begin{align*}
\norm{-\laplacian h_n}_{0,p} = 2 \norm*{N'_n + F(v + h_n) +
\frac{2\pi (k_+ - k_-)}{\abs\surface}}_{0,p} \to 0.
\end{align*}

Therefore, by the elliptic estimates and Sobolev's embedding,
$\norm{h_n - \avh_n}_{C^1} \to 0$. Finally, from the uniform bound
\eqref{eq:N'-bound}, $-(1 + \tau) \leq \bar N'_n \leq (1 - \tau)$ for
each $N'_n$, hence in the limit 
%
\begin{equation*}
  -(1 + \tau) \leq \bar N'_0 \leq 1 - \tau.
\end{equation*}

If $k_+ > k_-$, we rule out the possibility $\avh_n \to \infty$ and
similarly if $k_+ < k_-$.


\subsection{Multiple solutions in the unbalanced case}


Unlike the euclidean case, in a compact manifold there are multiple
solutions of the field equations if $k_+\neq k_-$. This was proved in
\cite{chiacchio2007multiple} for a related model together with bounds
for the constants in \cite{han2014multiplicity}. However their proofs
depend on the existence of a variable coupling constant $q$ for the
neutral field which in our case is fixed at $q = 1$. We will prove the
existence of multiple solutions to the field equations in the
unbalanced case, which can be seen in figure~\ref{fig:sols} on the
right column adapting the argument from \cite{chiacchio2007multiple}
to our restricted case. We will assume $k_+ < k_-$ in order to define
the positive constant $A = -4\pi(k_+ - k_-)/\abs\surface$, however the case
$k_+ > k_-$ can be treated similarly. Given $\kappa >
0$, let us define the functional $\Ik: \Hsp^2 \to \reals$, as

\begin{multline*}
\Ik(h) = \half\,\norm{\laplacian h}^2 + 2 \lproduct{F'(v + h), \abs{d(v +
  h)}^2} + 2 \norm{F(v + h)}^2 \\
+ \kappa^2 \brk(\half \norm{dh}^2  - A \lproduct{h, 1}),
\end{multline*}

where the norm and inner product appearing in the definition of $\Ik$
are defined in the $\Lsp^2$ sense. The following lemmas are
essentially the same as lemmas 1.2 and 1.3 in 
\cite{chiacchio2007multiple}, we refer the reader to such reference
for the proof. Recall solving equations \eqref{eq:h}-\eqref{eq:N}
is equivalent to solving \eqref{eq:h} and \eqref{eq:N'}.

\begin{lemma}\label{lem:weak-pair}
  A pair $(h, N') \in \Hsp^1\times \Hsp^1$ is a weak solution of
  equations \eqref{eq:h} and \eqref{eq:N'} if and only if $h
  \in \Hsp^2$ is a weak solution for the fourth order equation,
  %
  \begin{multline}
    \label{eq:fourth-order}
    \laplacian^2 h + \kappa^2\laplacian h = -2F''(v + h)\abs{d(v +
      h)}^2 -4\laplacian(F(v + h)) \\
    - 4 F'(v + h)F(v + h) + \kappa^2 A,
  \end{multline}
%
  and $N'$ is defined by,
  %
  \begin{equation}\label{eq:n'-from-h}
    N' = -\half\,(\laplacian h - A) - F(v + h).
  \end{equation}
\end{lemma}

\begin{lemma}\label{lem:weak-h2}
  $h \in \Hsp^2$ is a weak solution for \eqref{eq:fourth-order}
  if and only if it is a critical point for the $C^1$ functional $\Ik$. 
\end{lemma}

Hence, if we can find a critical point of $\Ik$,
lemma~\ref{lem:weak-pair} will give us a weak solution of the
elliptic problem, then by the usual bootstrap argument this weak
solution will be a smooth classical solution. Let $h_0$ be the unique
solution to equation \eqref{eq:h} for $\kappa = 0$ and let us fix a
constant $\mu < \min(\lproduct{h_0,1}, 0)$. We define the set,
%
\begin{equation*}
  \Aset = \set{h \in \Hsp^2 \mid h \leq \mu},
\end{equation*}
%
and note that if $h \in \Aset$, then $\Ik(h) \geq 0$. We also note
that $\Aset$ is closed and convex in $\Hsp^2$ and that for any $h \in \Aset$, by
Schauder's estimate and the fact that $\int h < 0$, we have
coercivity, i.e., there is a constant $C > 0$, such that,
%
\begin{equation*}
  \norm{h}_2^2 \leq C \Ik(h). 
\end{equation*}

Therefore, for any $\kappa \neq 0$, there is $h_{\kappa}\in\Aset$, such that
%
\begin{equation*}
  \Ik(h_{\kappa}) = \min_{\Aset} \Ik.
\end{equation*}

By Sobolev's embedding $\Hsp^2 \to C^0(\surface)$ and Sobolev's inequality,
%
\begin{equation*}
  \norm{h}_{C^0} \leq C \norm{h}_{\Hsp^2}, \qquad \forall h \in \Hsp^2,
\end{equation*}
%
if $h_{\kappa} < \mu$, there is an $\Hsp^2$ neighbourhood
of $h_{\kappa}$ contained in $\Aset$, hence $h_{\kappa}$ is a local
minimum in $\Hsp^2$ and by lemmas~\ref{lem:weak-pair}
and~\ref{lem:weak-h2}, we find smooth solutions to the 
elliptic problem. Since $\kappa$ is bounded, there is a constant such that,
%
\begin{equation*}
  0 \leq \Ik(h_{\kappa}) \leq C.
\end{equation*}

If we denote by $\bar h_{\kappa}$ the average of $h_{\kappa}$, by
Schauder's elliptic estimates, there is another constant such that, 
%
\begin{equation}
  \label{eq:ubound-hk-av}
  \norm{h_{\kappa} - \bar h_{\kappa}}^2_2 \leq C_1 \norm{\laplacian h}^2 \leq
  2 I_{\kappa}(k_{\kappa}) \leq 2C.
\end{equation}

Hence, the family of functions $\set{h_{\kappa} - \avh_{\kappa}}$ is uniformly
bounded by Sobolev's embedding.

\begin{lemma}\label{lem:av-div}
  The limit $\lim_{\kappa \to 0} \avh_{\kappa} = -\infty$ holds.
\end{lemma}

\begin{proof}
  We will prove the limit by proving that for any sequence $\kappa_n
  \to 0$, there exists a subsequence of $\avh_n = \avh_{\kappa_n}$,
  still denoted as $\avh_n$, such that $\avh_n\to -\infty$. Assume
  otherwise towards a contradiction, then there exists a bounded
  sequence $\set{\avh_n}$. After passing to a subsequence, we can
  assume $h_n$ converges weakly to some
  $h_0$ in $\Hsp^2$ by Alouglu's theorem and strongly in $\Lsp^2$ and
  $\Hsp^1$ by Rellich-Kondrachov's theorem applied to $h_n$ and
  $dh_n$. Hence, we also have the convergence $\avh_n \to \avh_0$ by
  the continuous embedding $\Lsp^2 \to \Lsp^1$. Since
  $\norm{\laplacian h_n}$ is bounded, we assume the convergence $\norm
  {\laplacian h_n}^2 \to 2 \alpha$. By the strong convergence of $h_n$ and
  $dh_n$, we have the limit,
  %
  \begin{equation*}
    \lim I_{\kappa_n}(h_n) = \alpha + 2 \lproduct{F'(v + h_0), \abs{dv +
        dh_0}^2} + 2 \norm{F(v + h_0)}^2.
  \end{equation*}
  
  From the definition of $I_{\kappa}$ we have $I_0(h) \leq
  I_{\kappa_n}(h)$ for any $h \in \Aset$, since $h$ is a negative
  function. Therefore,
  %
  \begin{equation*}
    \inf_\Aset I_0 \leq \lim I_{\kappa_n}(h_n).
  \end{equation*}

  On the other hand, 
  %
  \begin{align*}
    I_{\kappa_n}(h_n) &\leq I_{\kappa_n}(h) 
    = I_0(h) + \kappa \brk(\half \norm{dh}^2 - A \lproduct{h, 1}),
  \end{align*}
  %
  hence, $\lim I_{\kappa_n}(h_n) \leq I_0(h)$ for any $h \in \Aset$,
  from which we conclude
  %
  \begin{equation*}
   \lim I_{\kappa_n}(h_n) \leq \inf_\Aset I_0. 
  \end{equation*}

  Therefore $\inf_\Aset I_0 = \lim I_{\kappa_n}(h_n)$. Now we note
  that for a constant function $h(x) = c \in \Aset$, we have,
  %
  \begin{equation*}
    I_0(c) = 2\lproduct{F'(v + c), \abs{dv}^2} + 2\, \norm{F(v + c)}^2.
  \end{equation*}

  By the dominated convergence theorem,
  %
  \begin{equation*}
    \lim_{c \to - \infty} \lproduct{F'(v + c), \abs{dv}^2} = 0.
  \end{equation*}
  %
  Since $h_n \to h_0$ in $\Lsp^2$, we have $h_n \to h_0$ almost
  everywhere. Let $\epsilon > 0$, by Egorov's theorem, there exists a
  measurable set $\Omega$ of measure $\int_\Omega dV < \epsilon$ such
  that $h_n$ converges uniformly to $h_0$ in the complement
  $\surface\setminus \Omega$. Since each $h_n$ is continuous, $h_0$ is
  also continuous in $\surface \setminus \Omega$. If $c \leq
  c_\epsilon = \min_{\surface\setminus\Omega} h_0$, we have $v + c
  \leq v + c_\epsilon$ a.e., hence,
  % 
  \begin{align*}
    \norm{F(v + c)}^2 &\leq \norm{F(v + c_\epsilon)}^2 \\
                      &\leq \int_{\surface\setminus\Omega}F(v +
                        h_0)^2dV + \epsilon \max\set{1\pm \tau}\\
                      &\leq \norm{F(v + h_0)}^2 + \epsilon
                        \max\set{1\pm \tau}.
  \end{align*}

  We conclude the limit,
  %
  \begin{equation*}
    \lim_{c \to -\infty}\norm{F(v + c)}^2 \leq \norm{F(v + h_0)}^2,   
  \end{equation*}
  %
  and if $c$ is sufficiently small, 
  %
  \begin{equation*}
    I_0(c) \leq \lim I_{\kappa_n}(h_n) = \inf_\Aset I_0,
  \end{equation*}
  %
  hence $I_0(c) = \inf_\Aset I_0$, with $c < \mu$ so that the constant
  function $h(x) = c$ is a minimizer of $I_0$ in $\Hsp^2$ and
  therefore a solution of the regularised elliptic problem for the
  vortex-antivortex system at $\kappa = 0$ which is impossible.  
  This concludes the contradiction.
\end{proof} 

  By \eqref{eq:ubound-hk-av} and Sobolev's embedding, the
  family of continuous function $\set{h_\kappa - \avh_\kappa}$ is
  uniformly bounded and by lemma~\ref{lem:av-div}, if $\abs\kappa$ is
  small we have $h_\kappa < \mu$, hence by Sobolev's inequality, $h_\kappa$
  is a local minimizer of $I_\kappa$ in $\Hsp^2$. Finally, by lemmas
  \ref{lem:weak-pair}-\ref{lem:weak-h2} and the usual bootstrap
  argument, $h_\kappa$ and $N'_\kappa$ as defined in equation
  \eqref{eq:N'} are smooth solutions of the regularised elliptic
  problem. Since $h_{\kappa} \to -\infty$ as $\kappa \to 0$, for
  sufficiently small $\kappa$ these solutions are different of the
  pair $(k_{\kappa}, N'_{\kappa})$ found in
  section~\ref{sec:small-deform}. This result coincides with
  the result found by Chiacchio and Ricciardi 
  \cite{chiacchio2007multiple} using the variational approach and with
  another result by Han and Song \cite{han2011existence} using
  Schauder's degree theory.

  \subsection{Limit points as $\kappa \to
    0$}\label{sec:limit-points-kappa-0} 

  
  We consider the set,
  %
  \begin{equation*}
    \Kset = \set{ (h_\kappa, N'_\kappa) \mid \kappa > 0}.
  \end{equation*}
  %
  of solutions to the elliptic problem for $\kappa > 0$. We know
  $N'_\kappa$ is uniformly bounded by equation \eqref{eq:N'}. By
  \eqref{eq:h}, $\laplacian h_\kappa$ is bounded in $\Lsp^p$ for any
  $p \geq 2$. Therefore, by Sobolev's embedding, $\set{h_\kappa -
    \avh_\kappa}$ is uniformly bounded in $C^1$.

  \begin{lemma}
    For any converging sequence $(h_{\kappa_n} - \bar h_{\kappa_n},
    N'_{\kappa_n})$ with $\kappa_n \to 0$, we have either $\bar
    h_{\kappa_n} \to 0$ or $\bar h_{\kappa_n} \to \mp \infty$. In the
    first case, $\bar N'_{\kappa_n} \to 0$ whereas in the second case
    $\bar N'_{\kappa_n} \to 1 \mp \tau - \frac{2\pi (k_+ -
      k_-)}{\abs\surface}$. In both cases the sign in the second
    of convergence is determined by the sign of $k_+ - k_-$. 
  \end{lemma}

  \begin{proof}
    Let  $h_n = h_{\kappa_n}$, $N'_n = N'_{\kappa_n}$, and let us
    assume $\bar h_n \not\to 0$, from equation \eqref{eq:N'},
    %
    \begin{equation*}
      \kappa^2 \bar N'_n + 2 \lproduct{F'(v + h_n), N'_n} +
      \kappa^2\lproduct{ F(v + h_n), 1} = 0.
    \end{equation*}
    
  \end{proof}
  
  \begin{lemma}
    The only accumulation point of $\Kset$ in $\Hsp^2$ with $\kappa =
    0$ is $(h_0, 0)$, the solution to the vortex-antivortex elliptic
    problem, if we consider the set $\set{(h_\kappa, N'_\kappa - \bar
      N'_\kappa)}$ of solutions with $N'$ averaged to zero, then $(0,
    0)$ is also an accumulation point. In both cases, the convergence
    is $C^1$ uniform. 
  \end{lemma}
  
  \begin{proof}
    Let $\set{(h_n, N'_n)} \subset \Kset$ be any sequence in $\Kset$,
    
  \end{proof}


\section*{An index theorem}




  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let \ux \undefined
\let \ox \undefined

\let\Ik\undefined
\let\Aset\undefined
\let\avh\undefined
\let\Kset\undefined
%%% end-local %%%%%%%%%%%%%%%%%%%%%%





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../abelian-cs-deformation"
%%% End:


==> chapters/cs-term/abelian-deformations/sections/bounds2.tex <==
%%%% LOCAL LaTeX %%%%%%%%%%%%%%%%%%
\newcommand*\ux{\underline x}
\newcommand*\ox{\overline x}

\newcommand*\Ik{I_{\kappa}}
\newcommand*\Aset{\mathcal{A}}
\newcommand*\avh{\overline{h}}
\newcommand*\Kset{\mathcal{K}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{The unbalanced case}

We prove some necessary conditions for the solution of the elliptic
problem to exist. In this section we assume $k_+ \neq k_-$. Let $N' =
\kappa N$, equation~~\eqref{eq:N} can be rewritten as, 
%
\begin{equation}
  \label{eq:N'}
  \laplacian N' + (\kappa^2 + 2F'(v + h))\,N' + \kappa^2F(v + h) = 0.
\end{equation}

Let $\ux = \min_{\surface} \set{N'(x)}$, $\ox = \max_{\surface}\set{
  N' }$, if we denote by $F(x) = F(v(x) + h(x))$ and $F'(x) = F'(v(x)
+ h(x))$, by the maximum principle,
%
\begin{align*}
-\frac{\kappa^2F(\ux)}{\kappa^2 + 2F'(\ux)} \leq
N'(x) \leq
- \frac{\kappa^2 F(\ox)}{\kappa^2 + 2F'(\ox)}.
\end{align*}

Since $F'(x) \geq 0$, we conclude the uniform bounds,
%
\begin{align}\label{eq:N'-bound}
-(1 + \tau) \leq N' \leq (1 - \tau).
\end{align}

From equations \eqref{eq:h}  and \eqref{eq:N'} we obtain,
%
\begin{align*}
\laplacian N'- \frac{\kappa^2}{2} \brk(\laplacian h + \frac{4\pi}{\abs
\surface} (k_+ - k_-)) + 2F'(v + h)N' = 0. 
\end{align*}

Integrating this equation,
%
\begin{align*}
-2\pi\kappa^2(k_+ - k_-) + 2 \lproduct{F'(v + h), N'} = 0.
\end{align*}

Using the fact that $F'$ is a positive function bounded by
$1/2$ and the uniform bound for $N'$,
%
\begin{equation*}
\kappa^2 = \frac{\lproduct{F'(v + h), N'}}{\pi(k_+ - k_-)}
  \leq \frac{\max\set{1 \mp \tau} \abs\surface}{2\pi\abs{k_+ - k_-}}.
\end{equation*}

Therefore, the family of deformation constants is bounded, contrasting with the
ecuclidean case, in which there are cases for which the elliptic
problem can be solved for any $\kappa$ \cite{chen2019analysis}. We
will denote by $C$ a positive constant 
that can change from one equation to the other, from \eqref{eq:N'} we
have a uniform bound for the norm of $N'$ in Sobolev's space, 
%
\begin{equation*}
  \norm{\laplacian N'}_{0,p} \leq C(p), \qquad p \geq 2.
\end{equation*}

By Calderon-Sygmund theory, this implies,
%
\begin{equation*}
  \norm{N'}_{2,p} \leq C \brk(
  \norm{\laplacian N'}_{0,p} + \norm{N'}_{0,p}
  ) \leq C.
\end{equation*}

If we fix any $p > 2$, Sobolev's theory says that the embedding
$\Wsp(2, p) \to C^1(\surface)$ is continuous, then there 
exist constants independent of $\kappa$, such that,
%
\begin{equation*}
  \norm{N'}_{C^1} \leq C_1\norm{N'}_{2, p} \leq C_2.
\end{equation*}

Similarly, if $\avh = \lproduct{h, 1}/\abs\surface$ is
the average of a solution $h$ to \eqref{eq:h}, then the set
$\set{h_{\kappa} - \avh_{\kappa}}$, where $h_{\kappa}$ is a solution for any given
parameter $\kappa$, is also uniformly bounded in $C^1$. 

\subsection{Limit points of solutions as $\kappa \to 0$}

Let $(h_n, N'_n)$ denote a sequence of solutions to the
elliptic equations \eqref{eq:h}-\eqref{eq:N'} with a corresponding
sequence of parameters $\set{\kappa_n}$. We are interested in
describing the behaviour of these solutions as $\kappa_n \to 0$. We can
not rule out the possibility that $\avh_n \to \pm \infty$,
therefore, we assume firstly that $h_n - \avh_n \to
\tilde h$ and $N'_n \to N'_0$ in $\Hsp^1$ as $\kappa_n \to 0$. We
distinguish two cases. First, if $\avh_n \to c$ for some real number
$c$, then $h_n \to h_0$ in $\Hsp^1$, where $h_0 = \tilde h + c$. In
this case, $(h_0, N'_0)$ is a weak solution of \eqref{eq:h},
\eqref{eq:N'} with $\kappa = 0$, by elliptic theory, they are also a
classical solution of the equations, but we know that for $\kappa = 0$
the equations describe the vortex-antivortex situation in which case 
uniqueness implies that $N'_0 \equiv 0$ and $h_0$ is the only solution of
the regularised vortex-antivortex equation,
%
\begin{equation*}
  \laplacian h_0 + 2 F(v + h_0) + \frac{4\pi}{\abs\surface} (k_+ -
  k_-) = 0.
\end{equation*}

For the second case, let us assume $\avh_n \to \pm \infty$, from
equation \eqref{eq:h},
%
\begin{equation*}
  \bar N'_n \abs\surface + \lproduct{F(v + h_n), 1} + 2\pi(k_+ - k_-)
  = 0.
\end{equation*}

Since $N'_n \to N'_0$ in $\Lsp^2$, we have the convergence $\bar N'_n
\to \bar N'_0$ and since $h_n - \avh_n$ is uniformly bounded, by the
dominated convergence theorem,
%
\begin{equation*}
 \lproduct{F(v + h_n), 1} \to (\pm 1 + \tau)\abs\surface.
\end{equation*}

Hence, $\bar N'_0 = \mp 1 - \tau - \frac{2\pi (k_+ -
  k_-)}{\abs\surface}$. Since $F(v + h_n)$ is bounded for any $h_n$,
 $F'(v + h_n) \to 0$ pointwise and $N'_n$ is uniformly bounded, we
 deduce by \eqref{eq:N'}  and the dominated convergence theorem, that
 $\norm{\laplacian N'_n}_{0, p} \to 0$ for any $p > 2$. Therefore, by
 Schauder's estimates and Sobolev's embedding, we deduce that,
 %
 \begin{equation*}
   \norm*{N'_n - \brk(\mp 1 - \tau - \frac{2\pi(k_+ -
       k_-)}{\abs\surface})}_{C^1} \to 0.
 \end{equation*}

 Now, from \eqref{eq:h} we have,
 %
 \begin{align*}
\norm{-\laplacian h_n}_{0,p} = 2 \norm*{N'_n + F(v + h_n) +
\frac{2\pi (k_+ - k_-)}{\abs\surface}}_{0,p} \to 0.
\end{align*}

Therefore, by the elliptic estimates and Sobolev's embedding,
$\norm{h_n - \avh_n}_{C^1} \to 0$. Finally, from the uniform bound
\eqref{eq:N'-bound}, $-(1 + \tau) \leq \bar N'_n \leq (1 - \tau)$ for
each $N'_n$, hence in the limit 
%
\begin{equation*}
  -(1 + \tau) \leq \bar N'_0 \leq 1 - \tau.
\end{equation*}

If $k_+ > k_-$, we rule out the possibility $\avh_n \to \infty$ and
similarly if $k_+ < k_-$.


\subsection{Multiple solutions in the unbalanced case}


Unlike the euclidean case, in a compact manifold there are multiple
solutions of the field equations if $k_+\neq k_-$. This was proved in
\cite{chiacchio2007multiple} for a related model together with bounds
for the constants in \cite{han2014multiplicity}. However their proofs
depend on the existence of a variable coupling constant $q$ for the
neutral field which in our case is fixed at $q = 1$. We will prove the
existence of multiple solutions to the field equations in the
unbalanced case, which can be seen in figure~\ref{fig:sols} on the
right column adapting the argument from \cite{chiacchio2007multiple}
to our restricted case. We will assume $k_+ < k_-$ in order to define
the positive constant $A = -4\pi(k_+ - k_-)/\abs\surface$, however the case
$k_+ > k_-$ can be treated similarly. Given $\kappa >
0$, let us define the functional $\Ik: \Hsp^2 \to \reals$, as

\begin{multline*}
\Ik(h) = \half\,\norm{\laplacian h}^2 + 2 \lproduct{F'(v + h), \abs{d(v +
  h)}^2} + 2 \norm{F(v + h)}^2 \\
+ \kappa^2 \brk(\half \norm{dh}^2  - A \lproduct{h, 1}),
\end{multline*}

where the norm and inner product appearing in the definition of $\Ik$
are defined in the $\Lsp^2$ sense. The following lemmas are
essentially the same as lemmas 1.2 and 1.3 in 
\cite{chiacchio2007multiple}, we refer the reader to such reference
for the proof. Recall solving equations \eqref{eq:h}-\eqref{eq:N}
is equivalent to solving \eqref{eq:h} and \eqref{eq:N'}.

\begin{lemma}\label{lem:weak-pair}
  A pair $(h, N') \in \Hsp^1\times \Hsp^1$ is a weak solution of
  equations \eqref{eq:h} and \eqref{eq:N'} if and only if $h
  \in \Hsp^2$ is a weak solution for the fourth order equation,
  %
  \begin{multline}
    \label{eq:fourth-order}
    \laplacian^2 h + \kappa^2\laplacian h = -2F''(v + h)\abs{d(v +
      h)}^2 -4\laplacian(F(v + h)) \\
    - 4 F'(v + h)F(v + h) + \kappa^2 A,
  \end{multline}
%
  and $N'$ is defined by,
  %
  \begin{equation}\label{eq:n'-from-h}
    N' = -\half\,(\laplacian h - A) - F(v + h).
  \end{equation}
\end{lemma}

\begin{lemma}\label{lem:weak-h2}
  $h \in \Hsp^2$ is a weak solution for \eqref{eq:fourth-order}
  if and only if it is a critical point for the $C^1$ functional $\Ik$. 
\end{lemma}

Hence, if we can find a critical point of $\Ik$,
lemma~\ref{lem:weak-pair} will give us a weak solution of the
elliptic problem, then by the usual bootstrap argument this weak
solution will be a smooth classical solution. Let $h_0$ be the unique
solution to equation \eqref{eq:h} for $\kappa = 0$ and let us fix a
constant $\mu < \min(\lproduct{h_0,1}, 0)$. We define the set,
%
\begin{equation*}
  \Aset = \set{h \in \Hsp^2 \mid h \leq \mu},
\end{equation*}
%
and note that if $h \in \Aset$, then $\Ik(h) \geq 0$. We also note
that $\Aset$ is closed and convex in $\Hsp^2$ and that for any $h \in \Aset$, by
Schauder's estimate and the fact that $\int h < 0$, we have
coercivity, i.e., there is a constant $C > 0$, such that,
%
\begin{equation*}
  \norm{h}_2^2 \leq C \Ik(h). 
\end{equation*}

Therefore, for any $\kappa \neq 0$, there is $h_{\kappa}\in\Aset$, such that
%
\begin{equation*}
  \Ik(h_{\kappa}) = \min_{\Aset} \Ik.
\end{equation*}

By Sobolev's embedding $\Hsp^2 \to C^0(\surface)$ and Sobolev's inequality,
%
\begin{equation*}
  \norm{h}_{C^0} \leq C \norm{h}_{\Hsp^2}, \qquad \forall h \in \Hsp^2,
\end{equation*}
%
if $h_{\kappa} < \mu$, there is an $\Hsp^2$ neighbourhood
of $h_{\kappa}$ contained in $\Aset$, hence $h_{\kappa}$ is a local
minimum in $\Hsp^2$ and by lemmas~\ref{lem:weak-pair}
and~\ref{lem:weak-h2}, we find smooth solutions to the 
elliptic problem. Since $\kappa$ is bounded, there is a constant such that,
%
\begin{equation*}
  0 \leq \Ik(h_{\kappa}) \leq C.
\end{equation*}

If we denote by $\bar h_{\kappa}$ the average of $h_{\kappa}$, by
Schauder's elliptic estimates, there is another constant such that, 
%
\begin{equation}
  \label{eq:ubound-hk-av}
  \norm{h_{\kappa} - \bar h_{\kappa}}^2_2 \leq C_1 \norm{\laplacian h}^2 \leq
  2 I_{\kappa}(k_{\kappa}) \leq 2C.
\end{equation}

Hence, the family of functions $\set{h_{\kappa} - \avh_{\kappa}}$ is uniformly
bounded by Sobolev's embedding.

\begin{lemma}\label{lem:av-div}
  The limit $\lim_{\kappa \to 0} \avh_{\kappa} = -\infty$ holds.
\end{lemma}

\begin{proof}
  We will prove the limit by proving that for any sequence $\kappa_n
  \to 0$, there exists a subsequence of $\avh_n = \avh_{\kappa_n}$,
  still denoted as $\avh_n$, such that $\avh_n\to -\infty$. Assume
  otherwise towards a contradiction, then there exists a bounded
  sequence $\set{\avh_n}$. After passing to a subsequence, we can
  assume $h_n$ converges weakly to some
  $h_0$ in $\Hsp^2$ by Alouglu's theorem and strongly in $\Lsp^2$ and
  $\Hsp^1$ by Rellich-Kondrachov's theorem applied to $h_n$ and
  $dh_n$. Hence, we also have the convergence $\avh_n \to \avh_0$ by
  the continuous embedding $\Lsp^2 \to \Lsp^1$. Since
  $\norm{\laplacian h_n}$ is bounded, we assume the convergence $\norm
  {\laplacian h_n}^2 \to 2 \alpha$. By the strong convergence of $h_n$ and
  $dh_n$, we have the limit,
  %
  \begin{equation*}
    \lim I_{\kappa_n}(h_n) = \alpha + 2 \lproduct{F'(v + h_0), \abs{dv +
        dh_0}^2} + 2 \norm{F(v + h_0)}^2.
  \end{equation*}
  
  From the definition of $I_{\kappa}$ we have $I_0(h) \leq
  I_{\kappa_n}(h)$ for any $h \in \Aset$, since $h$ is a negative
  function. Therefore,
  %
  \begin{equation*}
    \inf_\Aset I_0 \leq \lim I_{\kappa_n}(h_n).
  \end{equation*}

  On the other hand, 
  %
  \begin{align*}
    I_{\kappa_n}(h_n) &\leq I_{\kappa_n}(h) 
    = I_0(h) + \kappa \brk(\half \norm{dh}^2 - A \lproduct{h, 1}),
  \end{align*}
  %
  hence, $\lim I_{\kappa_n}(h_n) \leq I_0(h)$ for any $h \in \Aset$,
  from which we conclude
  %
  \begin{equation*}
   \lim I_{\kappa_n}(h_n) \leq \inf_\Aset I_0. 
  \end{equation*}

  Therefore $\inf_\Aset I_0 = \lim I_{\kappa_n}(h_n)$. Now we note
  that for a constant function $h(x) = c \in \Aset$, we have,
  %
  \begin{equation*}
    I_0(c) = 2\lproduct{F'(v + c), \abs{dv}^2} + 2\, \norm{F(v + c)}^2.
  \end{equation*}

  By the dominated convergence theorem,
  %
  \begin{equation*}
    \lim_{c \to - \infty} \lproduct{F'(v + c), \abs{dv}^2} = 0.
  \end{equation*}
  %
  Since $h_n \to h_0$ in $\Lsp^2$, we have $h_n \to h_0$ almost
  everywhere. Let $\epsilon > 0$, by Egorov's theorem, there exists a
  measurable set $\Omega$ of measure $\int_\Omega dV < \epsilon$ such
  that $h_n$ converges uniformly to $h_0$ in the complement
  $\surface\setminus \Omega$. Since each $h_n$ is continuous, $h_0$ is
  also continuous in $\surface \setminus \Omega$. If $c \leq
  c_\epsilon = \min_{\surface\setminus\Omega} h_0$, we have $v + c
  \leq v + c_\epsilon$ a.e., hence,
  % 
  \begin{align*}
    \norm{F(v + c)}^2 &\leq \norm{F(v + c_\epsilon)}^2 \\
                      &\leq \int_{\surface\setminus\Omega}F(v +
                        h_0)^2dV + \epsilon \max\set{1\pm \tau}\\
                      &\leq \norm{F(v + h_0)}^2 + \epsilon
                        \max\set{1\pm \tau}.
  \end{align*}

  We conclude the limit,
  %
  \begin{equation*}
    \lim_{c \to -\infty}\norm{F(v + c)}^2 \leq \norm{F(v + h_0)}^2,   
  \end{equation*}
  %
  and if $c$ is sufficiently small, 
  %
  \begin{equation*}
    I_0(c) \leq \lim I_{\kappa_n}(h_n) = \inf_\Aset I_0,
  \end{equation*}
  %
  hence $I_0(c) = \inf_\Aset I_0$, with $c < \mu$ so that the constant
  function $h(x) = c$ is a minimizer of $I_0$ in $\Hsp^2$ and
  therefore a solution of the regularised elliptic problem for the
  vortex-antivortex system at $\kappa = 0$ which is impossible.  
  This concludes the contradiction.
\end{proof} 

  By \eqref{eq:ubound-hk-av} and Sobolev's embedding, the
  family of continuous function $\set{h_\kappa - \avh_\kappa}$ is
  uniformly bounded and by lemma~\ref{lem:av-div}, if $\abs\kappa$ is
  small we have $h_\kappa < \mu$, hence by Sobolev's inequality, $h_\kappa$
  is a local minimizer of $I_\kappa$ in $\Hsp^2$. Finally, by lemmas
  \ref{lem:weak-pair}-\ref{lem:weak-h2} and the usual bootstrap
  argument, $h_\kappa$ and $N'_\kappa$ as defined in equation
  \eqref{eq:N'} are smooth solutions of the regularised elliptic
  problem. Since $h_{\kappa} \to -\infty$ as $\kappa \to 0$, for
  sufficiently small $\kappa$ these solutions are different of the
  pair $(k_{\kappa}, N'_{\kappa})$ found in
  section~\ref{sec:small-deform}. This result coincides with
  the result found by Chiacchio and Ricciardi 
  \cite{chiacchio2007multiple} using the variational approach and with
  another result by Han and Song \cite{han2011existence} using
  Schauder's degree theory.

  \subsection{Limit points as $\kappa \to
    0$}\label{sec:limit-points-kappa-0} 

  
  We consider the set,
  %
  \begin{equation*}
    \Kset = \set{ (h_\kappa, N'_\kappa) \mid \kappa > 0}.
  \end{equation*}
  %
  of solutions to the elliptic problem for $\kappa > 0$. We know
  $N'_\kappa$ is uniformly bounded by equation \eqref{eq:N'}. By
  \eqref{eq:h}, $\laplacian h_\kappa$ is bounded in $\Lsp^p$ for any
  $p \geq 2$. Therefore, by Sobolev's embedding, $\set{h_\kappa -
    \avh_\kappa}$ is uniformly bounded in $C^1$.

  \begin{lemma}
    For any converging sequence $(h_{\kappa_n} - \bar h_{\kappa_n},
    N'_{\kappa_n})$ with $\kappa_n \to 0$, we have either $\bar
    h_{\kappa_n} \to 0$ or $\bar h_{\kappa_n} \to \mp \infty$. In the
    first case, $\bar N'_{\kappa_n} \to 0$ whereas in the second case
    $\bar N'_{\kappa_n} \to 1 \mp \tau - \frac{2\pi (k_+ -
      k_-)}{\abs\surface}$. In both cases the sign in the second
    of convergence is determined by the sign of $k_+ - k_-$. 
  \end{lemma}

  \begin{proof}
    Let  $h_n = h_{\kappa_n}$, $N'_n = N'_{\kappa_n}$, and let us
    assume $\bar h_n \not\to 0$, from equation \eqref{eq:N'},
    %
    \begin{equation*}
      \kappa^2 \bar N'_n + 2 \lproduct{F'(v + h_n), N'_n} +
      \kappa^2\lproduct{ F(v + h_n), 1} = 0.
    \end{equation*}
    
  \end{proof}
  
  \begin{lemma}
    The only accumulation point of $\Kset$ in $\Hsp^2$ with $\kappa =
    0$ is $(h_0, 0)$, the solution to the vortex-antivortex elliptic
    problem, if we consider the set $\set{(h_\kappa, N'_\kappa - \bar
      N'_\kappa)}$ of solutions with $N'$ averaged to zero, then $(0,
    0)$ is also an accumulation point. In both cases, the convergence
    is $C^1$ uniform. 
  \end{lemma}
  
  \begin{proof}
    Let $\set{(h_n, N'_n)} \subset \Kset$ be any sequence in $\Kset$,
    
  \end{proof}


\section*{An index theorem}




  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let \ux \undefined
\let \ox \undefined

\let\Ik\undefined
\let\Aset\undefined
\let\avh\undefined
\let\Kset\undefined
%%% end-local %%%%%%%%%%%%%%%%%%%%%%





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../abelian-cs-deformation"
%%% End:


==> chapters/cs-term/commands.tex <==
\usepackage{xparse}

%%% Miscelaneous maths

\NewDocumentCommand\set{m}{
  \left\{#1\right\}
}

\NewDocumentCommand\st{m}{
  \;\left\lvert\;{#1}\right.
}

\NewDocumentCommand\brk{r()}{
    \left( {#1} \right)
}

\newcommand*\half{\frac{1}{2}}




%%% Field theory

\def\higgsField{\phi}
\def\gaugePotential{a}
\def\electricField{e}
\def\magneticField{B}
\def\spacetimeGaugePotential{A}
\def\curvatureField{F}
\def\neutralField{N}
\def\fieldConfSpace{\mathcal{A}}
\def\gaugeTransfSpace{\mathcal{G}}
\def\configurationSpace{\mathscr{C}}
\def\bigTantent{\mathcal{T}}
\def\vertSpace{\mathcal{V}}
\def\connectionSpace{\mathscr{A}}
\def\gaugeTransfSpace{\mathscr{G}}
\def\LagrangianDensity{\mathcal{L}}

\newcommand*\hf{\higgsField}
\newcommand*\gp{\gaugePotential}
\newcommand*\ef{\electricField}
\newcommand*\mf{\magneticField}
\newcommand*\cf{\curvatureField}
\newcommand*\nf{\neutralField}
\newcommand*\confSp{\configurationSpace}
\newcommand*\gaugeSp{\gaugeTransfSpace}
\newcommand*\vertSp{\mathcal{V}}
\newcommand*\gaugeGp{\gaugeTransfSpace}
\newcommand*\fieldSp{\fieldConfSpace}
\newcommand*\connSp{\connectionSpace}
\newcommand*\connForm{\omega}
\newcommand*\bigTangent{\mathcal{T}}
\newcommand*\pair{\Phi}
\newcommand*\vset{\mathcal{P}}
\newcommand*\stgp{\spacetimeGaugePotential}
\newcommand*\hreg{\tilde h}
\newcommand*\htilde{\hreg}
\newcommand*\chireg{\tilde \chi}
\newcommand*\ConTr{\Omega_\moduliSp}

\DeclareMathOperator\Energy{E}
\DeclareMathOperator\KinEn{T}
\DeclareMathOperator\PotEn{V}
\DeclareMathOperator\KinTr{K}
\DeclareMathOperator\Lagrangian{L}
\DeclareMathOperator\LagDens{\LagrangianDensity}

%%% Geometry

\def\covariantDerivative{\nabla}


\newcommand*\vb{\mathbf}
\newcommand*\plane{{\R^2}}
\newcommand*\surface{\Sigma}
\newcommand*\sphere{\mathbb{S}^2}
\newcommand*\spacetime{\R^{1 + 2}}
\newcommand*\cdv{\covariantDerivative}
\newcommand*\vp{\mathbf{p}}
\newcommand*\conFc{\Omega}
\newcommand*\dist{\mathrm{d}}
\newcommand*\manifold{M}

\DeclareMathOperator\Aut{Aut}


%%% Analysis


\newcommand*\moduliSp{\mathcal{M}}
\newcommand*\eval[2]{\left. #1 \right\rvert_{#2}}
\newcommand*\laplacian{\Delta}
\newcommand*\slaplacian{\Delta_\surface}
\newcommand*\dvr[1]{\nabla\cdot\mathbf{#1}} %DiVeRgence
\newcommand*\grad{\nabla}
\newcommand*\del{\partial}
\newcommand*\Diff{\mathcal{D}}
\newcommand*\reals{\mathbb{R}}
\newcommand*\cpx{\mathbb{C}}
\newcommand*\R{\mathbb{R}}%
\newcommand*\C{\mathbb{C}}%
\newcommand*\conj[1]{\overline{#1}}
\newcommand*\disk{D}
\newcommand*\order{\mathcal{O}}
\newcommand*\vdel{\del}
\newcommand*\dTaubes{\del_v\!\TaubesOp}
\newcommand*\afn{a}
\newcommand*\bfn{b}
\newcommand*\ueps{u}
\newcommand*\Xsp{\mathcal{X}}
\newcommand*\hilbSp{\mathcal{H}}
\newcommand*\fFunc{\mathcal{F}}
\newcommand*\intManifold{\int_\manifold}
\newcommand*\Hn{\mathrm{H}}
\newcommand*\wto{\rightharpoonup}

\DeclareMathOperator\ElpOp{E}
\DeclareMathOperator\Lsp{L^2}
\DeclareMathOperator\Hsp{H}
\DeclareMathOperator\Reg{Reg}
\DeclareMathOperator\Arg{Arg}
\DeclareMathOperator\TaubesOp{L}

\NewDocumentCommand\lproduct{sm}{
  \IfBooleanTF#1
    {
        \left\langle{#2}\right\rangle
    }{
        \langle{#2}\rangle
    }
}

\NewDocumentCommand\pdv{mo}{
 % Example ussage:
 % \pdv{x}y  : This is the partial derivative operator "times" y.
 % \pdv{x}[y]: This is the partial derivative y with respect to x.
 \IfValueTF{#2}
 {\frac{\del #2}{\del #1}}
 {\frac{\del}{\del #1}}
}

\NewDocumentCommand\abs{sm}{
  \IfBooleanTF#1
  {
    \left\lvert {#2} \right\rvert}
  {
    \lvert {#2} \rvert
  }
}

\NewDocumentCommand\norm{sm}{
  \IfBooleanTF#1
  {
    \left\lvert\left\lvert {#2} \right\rvert\right\rvert
  }
  {
    \lvert\lvert {#2} \rvert\rvert
  }
}

\newcommand*\dv[1]{\frac{d}{d #1}}


%%% Algebra

\NewDocumentCommand\hprod{sm}{
  \IfBooleanTF#1
  {
    \left\langle {#2} \right\rangle
  }
  {
    \langle {#2} \rangle
  }
}


\newcommand*\aForm{B}

\DeclareMathOperator\Ker{Ker}
\DeclareMathOperator\Proj{\Pi}

%%% Local Variables:
%%% mode: plain-tex
%%% TeX-master: t
%%% End:


==> chapters/cs-term/sections/coeff-sym.tex <==

\section{Symmetries of the $b_p$ coefficients}
\label{sec:coeff-sym}

Here we prove the symmetry used to simplify the curvature form,
equation \eqref{eq:b-sym}. We follow
\cite[p.~209]{manton_topological_2004} and consider an $h$ to lowest
order in $\kappa$. If $\surface$ is the Euclidean
plane, we assume $h \to 0$ as $\abs{x} \to \infty$, on the
other hand, if $\surface$ is a compact surface, we assume $p, q \in
\vset$ lie in an open and dense subset $U$, homeomorphic to a disk in
which a coordinate system has been chosen such that the metric is
conformally flat. Let $\ElpOp = \laplacian_{\surface} - \abs\hf^2$, by
equation \eqref{eq:bog-h-lin}, $\del_ph$ is a Green's function of
$\ElpOp$. Let us assume $p \neq q$, we apply Green's second identity


\begin{align}
\label{eq:apx-green-id}
0 = \int_{\surface} (\del_qh \ElpOp \del_ph - \del_ph \ElpOp \del_qh) * 1
= -4\pi \brk(
\del\del_q h(p) - \del\del_p h(q)
).
\end{align}

Since $p \neq q$, we have,

\begin{equation}
\label{eq:del-delq-hp}
\del\del_q h(p) = \half \del_q\conj{b_p}.
\end{equation}

Similarly for $\del\del_ph(q)$, we conclude the symmetry

\begin{equation}
\label{eq:coeff-sym}
\del_q\conj{b_p} = \del_p\conj{b_q}.
\end{equation}

Similarly,

\begin{align}
\label{eq:apx-green-id-conj}
0 = \int_{\surface} (\conj{\del_q}h \ElpOp \del_ph - \del_ph \ElpOp
\conj{\del_q}h) * 1
= -4\pi \brk(
\del\conj{\del_q} h(p) - \conj\del\del_p h(q)
).
\end{align}

from which we have,

\begin{equation}
\label{eq:coeff-sym-conj}
\conj{\del_q}\conj{b_p} = \del_p b_q.
\end{equation}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../chern-simmons-loc.tex"
%%% End:


==> chapters/cs-term/sections/gf.tex <==
\section{Gauge freedom}
\label{sec:gauge-freedom}


In this section we specialise in a trivial fibber bundle $\plane
\times \C$, i.e., we will work in the setting of Ginzburg-Landau field
theory. Let us consider a pair $\pair \in \fieldSp$, such that $\hf$
and $\gp$ satisfy the first Bogomolny equation~\eqref{eq:bog}. Let
$\vset = \hf^{-1}(0)$ be the set of zeros of the Higgs field, $\hf$ is
a vortex solution if for each $p\in\vset$, the Higgs field has winding
number $2\pi$ about $p$, for any simple, closed curved
surrounding the point in a sufficiently small neighbourhood. Let us
define the functions $h, \chi:\plane\setminus\vset \to \R$, such that,

\begin{equation}
\label{eq:vortex-cart->polar}
\hf = e^{\frac{h}{2} + i\chi},
\end{equation}

$h$ is gauge independent, however $\chi$ is not, even worse,
$\chi$ is ill defined, in fact, there is a discrete family of possible
$\chi$ functions determining the same argument for
$\hf$. Nevertheless, $\chi$ is a differentiable function in each
branch of definition. On $\plane \setminus \vset$, equation~ 
\eqref{eq:bog} is equivalent to

\begin{equation}
\label{eq:gp-phase-rel}
A = d\chi - \half *dh,
\end{equation}

we also note that $h$ is gauge equivalent, whereas $\chi$ is not. From
equation \eqref{eq:gp-phase-rel}, $\chi$ is a solution on
$\plane\setminus\vset$ to the equation

\begin{equation}
\label{eq:chi-gov-elliptic}
\laplacian \chi = \dvr \gp.
\end{equation}

From equation \eqref{eq:gp-phase-rel} we can also compute the phase
$\chi$. For fixed $x_0\in\plane\setminus \vset$ but otherwise
arbitrary, let $\gamma: I \to \plane\setminus\vset$ be a continuous
curve starting at $x_0$, then

\begin{equation}
\label{eq:gp->phase}
\chi = \int_{\gamma} \left(\gp - \half *dh\right) + \chi(x_0), 
\end{equation}

$\chi$ is well defined up to multiples of $2\pi$ which account for the
number of times that $\gamma$ winds around each vortex position. If we
change the gauge, say by a function $\alpha:\plane\to\R$, then $\chi$
changes to $\chi + \alpha$, on the other hand, by equation
\eqref{eq:gp-phase-rel},

\begin{equation}
\label{eq:taubes}
\laplacian h = 2*d\gp,
\end{equation}

which is the, necessarily, gauge invariant equation satisfied by
$h$. The condition that $p$ is a single vortex translates into a
local statement about $\hf$. It means that $p$ is a simple zero of the
field. In turn, this means that both $h$ and $\chi$ have
logarithmically divergent singularities for each $p \in \vset$. In
order to 
have a complete description of the problem, we add the boundary
conditions

\begin{align}
\label{eq:bnd-cond-h}
\lim_{\abs{x} \to \infty} h &= 0, &
\lim_{\abs{x - p} \to 0} \abs*{\frac{h(x)}{\log\abs{x - p}}} &< \infty,
&
\lim_{\abs{x - p} \to 0} \abs*{\frac{\chi(x)}{\log\abs{x - p}}} &<
\infty, \qquad p \in \vset.
\end{align}


We deduce from equations~\eqref{eq:gl-perp-cond}~and~
\eqref{eq:chi-gov-elliptic}, the relation,

\begin{equation}
\label{eq:beta->chi}
\left( \laplacian - e^h \right)(\beta - \dot\chi) = 0.
\end{equation}


Equation~\eqref{eq:beta->chi} is gauge invariant, if $\alpha_s \in
\gaugeGp$ is a family of gauge transformations varying differentiably,
it is easy to check that $\beta$ has to be replaced by $\beta +
\dot\alpha$, just like $\dot\chi$, in order to keep gauge invariance. 
If $A_0:\plane \to \R$ is a smooth solution  to $(\laplacian -
\abs{\hf}^2) A_0 = 0$, of finite energy,

\begin{equation}
\label{eq:julia-zee-cond}
\int_{\plane} \abs{\grad A_0}^2 dx < \infty,
\end{equation}

and if $\hf$ is non-zero, then $A_0 = 0$. This is know as the
Julia-Zee theorem, it was stated by Julia and
Zee to prove that moving Ginzburg-Landau vortices are electrically
neutral \cite{julia-poles-1975}. Later, Spruck and Yang proved it
\cite{spruck-proof-2009}. For each $p \in \vset$, let $\theta_p(x) =
\Arg(x - p)$, the condition on each $p$ of being a single vortex
means that there exists a continuous function $\tilde\chi$ such that,

\begin{equation}
\label{eq:argument-reg-part}
\chi = \sum_{p \in \vset} \theta_p + \tilde\chi,
\end{equation}

$\tilde\chi$ is the regular part of $\chi$, which will be denoted as
$\Reg(\chi)$. Let $\Theta = \sum_{p\in\vset} \theta_p$, then $\Theta$
is the singular part of the argument field and up to gauge
equivalence. By the Julia-Zee theorem, $\chi$ is basically the sum of
the arguments with respect to the points in the vortex set. To end
this section, we quote the singular and regular part of $\dot\chi$, 

\begin{equation}
\label{eq:dot-argument-reg-part}
\dot\chi = \sum_{p\in\vset} -\frac{1}{2i} \left(
  \frac{\dot p}{x - p} - \frac{\dot p^{\dagger}}{(x - p)^{\dagger}}
\right) + \Reg\dot\chi.
\end{equation}








%%% Local Variables:
%%% TeX-master: "../chern-simmons-loc.tex"
%%% End:


==> chapters/cs-term/sections/linear-prob.tex <==

\section{Linear elliptic problems}
\label{sec:line-ellipt-probl}


In this section we prove a result about existence of solutions of
linear elliptic equations in a compact manifold. We state the result
as a lemma.

\begin{lemma}
  \label{lem:linear-prob-cmp}
If $\manifold$ is a compact Riemannian manifold of dimension
$n$, $\laplacian_{\manifold}$  is the Laplace-Beltrami operator of the
metric, $\afn, \bfn \in \Lsp(\manifold)$ are functions such that
$\afn$ is non-negative and bounded with positive integral $\int_M \afn
*1$, then the problem, 

\begin{equation}
  \label{eq:linear-problem}
  -\laplacian \ueps = \afn\ueps + \bfn.
\end{equation}

has exactly one solution $\ueps \in \Hsp^2(\manifold)$. Moreover,
there is a positive constant $C$ such that,

\begin{equation}
  \label{eq:linear-bound-lem-cmp}
  \norm{\ueps}_2 \leq \norm{\afn}_0\cdot
  K + \norm{\bfn}_0.
\end{equation}
\end{lemma}

If $n = 2, 3$, by Sobolev's embedding, $\ueps \in C^0(\manifold)$, in
general, we only have $\ueps \in \Hsp^2(\manifold)$ unless we know
that $\afn$ and $\bfn$ have more regularity. This problem has been
studied for different conditions on the coefficients 
\cite{mitrea1999boundary,mitrea2000potential}, the version we state in
lemma \ref{lem:linear-prob-cmp} suits the hypothesis used in section
\ref{sec:comp-case} to prove regularity of the dependence on
parameters of $\htilde$ the regular part of the solution to Taubes'
equation.  We will prove the 
existence of solutions to equation \eqref{eq:linear-problem} and continuity of 
the datum as an application of Lax-Milgram's theorem. 

Let $\Xsp$ be the subspace of $\Hsp^1 (\manifold)$ of
functions of zero average, 

\begin{equation}
  \label{eq:Xsp-def-manifold}
  \Xsp =
   \set{ u \in \Hsp^1(\manifold) \st \int_M u *1 = 0}.
\end{equation}

$\Hsp^1 (\manifold)$ can be decomposed as

\begin{equation}
  \label{eq:cann-decomp-manifold}
  \Hsp^1 (\manifold) = \Xsp \oplus \reals.
\end{equation}

Equation \eqref{eq:linear-problem} is equivalent to finding 
$(\ueps_0, c) \in\Xsp \oplus \reals$, such that

\begin{equation}
  \label{eq:linear-prob-h10}
  -\laplacian \ueps_0 = \afn\ueps_0 + \afn\,c + \bfn.
\end{equation}

By the divergence theorem, the constant is


\begin{equation}
  \label{eq:c-value}
  c = \frac{
   -\int_{\manifold} (\afn\ueps_0 + \bfn) *1
  }{
   \int_{\manifold}\afn *1
  }.
\end{equation}

\eqref{eq:linear-problem} is equivalent to finding $\ueps_0 \in \Xsp$ such that

\begin{equation}
  \label{eq:h10-equiv-problem}
  -\laplacian\, \ueps_0 = \afn\ueps_0 + \bfn - \frac{
    \afn \cdot \int_{\manifold} (\afn\ueps_0 + \bfn) *1
  }{
    \int_{\manifold}\afn *1
  }.
\end{equation}

Let us define the operators $\aForm:\Xsp\times\Xsp \to \reals$, $\fFunc:
\Xsp \to \reals$, as

\begin{align}
\aForm(u, v) &= \lproduct{ d\ueps, dv} + \lproduct{\afn\ueps, v}
  - \frac{1}{\intManifold\afn *1}\,
   \intManifold \afn \ueps *1 \cdot\intManifold \afn v *1,\\
\fFunc(v) &=
\frac{
    1
  }{
    \intManifold\afn *1
  }
  \intManifold
  \left(
    \afn\cdot\intManifold\bfn *1 - \bfn \cdot\intManifold\afn *1
  \right)\cdot v *1. 
\end{align}

Equation (\ref{eq:h10-equiv-problem}) can be rewritten in variational
form as the problem of finding $\ueps_0 \in\Xsp$, such that for any $v
\in \Xsp$,

\begin{equation}
  \label{eq:variational-problem}
  \aForm(\ueps_0, v) = \fFunc(v).
\end{equation}

$\fFunc$ is bounded and $\aForm$ continuous because
$\afn, \bfn \in \Lsp^2(\manifold)$. By Cauchy-Schwartz's inequality,

\begin{equation}
  \label{eq:cauchy-schwartz}
  \abs*{\intManifold \afn \ueps\, \vform} \leq
  \norm{\sqrt\afn}_0\,\norm{\sqrt\afn\ueps}_0,
\end{equation}

hence,

\begin{equation}
  \label{eq:a-bil-coercive}
  \begin{aligned}[b]
      \aForm(u, u) &= \norm{d\ueps}^2_0
  + \frac{
    1
  }{
    \intManifold a *1
  } \brk(
    \intManifold a \ueps^2 *1 \cdot \intManifold a *1
    -  \brk( \intManifold a\ueps *1)^2
    )\\
   &= \norm{d\ueps}^2_0 + \frac{
    1
  }{
    \intManifold a *1
  } \brk( 
    \norm{\sqrt{\afn} u}^2_0\,\norm{\sqrt\afn}^2_0 - \lproduct{\afn, u}^2_0
  )\\
   &\geq \norm{d\ueps}^2_0.
  \end{aligned}
  \end{equation}

  By Poincar\'e's inequality, there is a positive
  constant $\alpha$, such that

  \begin{equation}
    \label{coercivity-A-H10}
    \alpha\,\norm{\ueps}_1^2 \leq 
    \norm{d\ueps}^2_0 \leq  \aForm(\ueps, \ueps). 
  \end{equation}

 Therefore, there exists a unique solution $\ueps \in
\Hsp^1 (\manifold)$ to \eqref{eq:linear-problem}. By standard elliptic
regularity estimates, $u \in \Hsp^2(\manifold)$. By Lax-Milgram's theorem,

\begin{equation}
  \label{eq:u0-F-bound}
  \norm{\ueps_0}_1 \leq \frac{
    1
  }{
    \alpha\intManifold a *1
  }\,\norm*{
    a\cdot\intManifold b *1 - b\cdot\intManifold a *1
  }_0. 
\end{equation}

By equation~(\ref{eq:c-value}),

\begin{equation}
  \label{eq:c-bound}
  \abs{c} \leq \frac{
    1
  }{
    \intManifold \afn *1
  } \brk(
    \norm{\afn}_0\cdot \norm{\ueps_0}_0 +
    \abs*{\intManifold b *1}
  ).
\end{equation}

Therefore, $\ueps$ is bounded in $\Hsp^1 (\manifold)$ by,

\begin{equation}
  \label{eq:u-bound}
  \norm{\ueps}_1 \leq
  \frac{
    C
  }{
    \intManifold \afn *1
  } \brk(
    \frac{
      \norm{\afn}_0^2
    }{
      \intManifold \afn *1
    }
    + \norm{\afn}_0
    + 1
  )
  \norm{\bfn}_0,
\end{equation}

for some suitable constant $C$. By the elliptic estimate for equation
(\ref{eq:linear-problem}) we conclude $\ueps \in \Hsp^2(\manifold)$.







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../../geometric-models.tex"
%%% End:


==> chapters/cs-term/sections/loc.tex <==
\section{Localisation }
\label{sec:cs-loc-formulas}



\subsection{An example: Strachan-Samols meromorphic localisation}
\label{sec:loc-formula-examples}

We will show two examples about how the localisation formula arises
from the general description we have made of moduli
space. Firstly, let us consider the Ginzburg-Landau functional. In
this case, the domain is the Euclidean plane, the principal bundle is the
trivial bundle $\plane \times U(1)$ and the structure group acts in the
model space, $\cpx$ canonically. Here, target space is also the
trivial bundle $\spacetime \times \cpx$, and the metric in space-time
has signature $(+,-,-)$. If $\hf : \spacetime \to \cpx$
is a section on target space, and $\stgp \in \Omega^1(\spacetime)$ is a
connection form, there is a way to define a covariant derivative
$\Diff\hf \in \Omega^1(\spacetime, \cpx)$, compatible with the action of the
structure group, 

\begin{equation}
\label{eq:gl-cov-der}
\Diff\hf = d\hf - i \hf\stgp,
\end{equation}

where we have identified tangent vectors with complex numbers in
target space. We will split $\stgp$ in its temporal ans spatial
components,

\begin{equation}
\label{eq:stgp-split}
\stgp = \gp_0dx^0 + \gp,
\end{equation}

where we think of the components as curves

\begin{align}
\label{eq:loc-stgp-split}
\gp_0:\reals \to
C^{\infty}(\plane), &&
\gp: \reals \to \Omega^1(\plane).
\end{align}

Likewise, we define the magnetic and
electric forms, $\mf:\reals \to \Omega^2(\plane)$ and $\ef:\reals \to
\Omega^1(\plane, \reals)$ respectively, as the components of the curvature form,

\begin{align}
\label{eq:loc-def-mf-ef}
d\stgp = -\ef\wedge dx^0 + \mf.
\end{align}

Bearing this settings in mind, the Ginzburb-Landau
functional for static fields in the radiation gauge, is

\begin{equation}
\label{eq:gl-functional}
\mathcal{L}_{\mathrm{GL}} = \half \left(\abs{\Diff\hf}^2  +
  \abs{d\stgp}^2\right) + \frac{\lambda}{4}
(1 - \abs\hf^2)^2.
\end{equation} 

The metric in $\Omega^1(\spacetime, \cpx)$ is the induced metric from
space-time. We wont delve into the details of Ginzburg-Landau
theory, but we remark that if $\lambda = 1$, and we take the radiation
gauge, where $\gp_0 = 0$, static
energy minimisers of \eqref{eq:gl-functional} in the radiation gauge
where the time component of $\stgp$ is null are solutions to
Bogomolny's equations \cite{bogomolny_stability_1976}, 

\begin{align}
\label{eq:bog}
\Diff_1\hf + i \Diff_2\hf &= 0, &
*\mf &= \half ( \abs\hf^2 - 1),
\end{align}

with the boundary conditions,

\begin{align}
\label{eq:bog-bd}
\lim_{\abs x \to \infty} \hf(x) &= 0, &
\lim_{\abs x \to \infty} *\mf &= 0.
\end{align}

The space of solutions of Bogomonly's equations
modulo gauge equivalence is a moduli space, depending on the set of
zeros $\vset$ of the Higgs field $\hf$, which can be proved is a
discrete subset of the plane \cite{taubes1980}. Let us
denote by $\fieldSp'$ the 
subset of $\fieldSp$ of solutions of Bogomlny's equations, and by
$\moduliSp$ its moduli space, $\fieldSp'/\gaugeGp$. Then,
we have a bundle inclusion,

\begin{equation}
  \label{eq:bundle-comm-diag}
\begin{tikzcd}
  \fieldSp' \arrow[d] \arrow[r, hook] & \fieldSp \arrow[d] \\
  \moduliSp             \arrow[r,hook]  & \confSp
\end{tikzcd}  
\end{equation}

and since Bogomolny's equations are gauge invariant, both bundles share
the same vertical space. Therefore, the orthogonal projection into
$\vertSp$ is the same in the space of solutions to Bogomolny's
equations. Hence $\beta$ is the projection of a variation $(\delta\hf,
\delta\gp)$ into vertical space, if and only if is a
solution to equation \eqref{eq:perp-condition}. If $(p_1, \ldots,
p_k)$ are the zeros of a field $\hf \in \fieldSp'$, and we let
the zeros vary with respect to a parameter, $p_k(s)$, identified as the
\emph{time} parameter, then equation \eqref{eq:perp-condition} is
equivalent to,

\begin{equation}
\label{eq:gl-perp-cond}
(\laplacian - \abs{\hf}^2)\beta = -\frac{i}{2} \left( \hf
  \dot\hf^{\dagger} - \dot\hf \hf^{\dagger} \right) + \dvr\gp,
\end{equation}

and therefore, projection of the variation in the horizontal subspace
of $\bigTangent$ is

\begin{align}
\label{eq:orth-complement}
\delta\hf^{\perp} &= \dot{\hf} - i\hf\beta, &
\delta\gp^{\perp} &= \dot\gp - d\beta.
\end{align}

Since the variation is determined by variations in the core $p_k$
positions, we know that,

\begin{align}
\label{eq:gl-var-core}
\dot\hf &= \dot p_k\, \pdv{p_k}[\hf], &
\dot\gp &= \dot p_k\, \pdv{p_k}[\gp] .
\end{align}

If $\beta_k$ is the solution to equation \eqref{eq:gl-perp-cond} for the
data $(\del_{p_k}\hf, \del_{p_k}\gp)$, then $\beta = \dot
p_k\,\beta_k$. Here, and in the sequel, we make the convention that
repeated indices represent sums.  If we denote the pair
$(\hf, \gp)$ by $\pair$, and take variations and orthogonal complement
component wise, the instant energy of a trajectory in moduli space is therefore,

\begin{align}
\nonumber
\Energy[\dot\pair] &= \half \norm{(\dot\hf,
  \dot\gp)}^2_{\fieldSp}  \\
  \nonumber
  &= \half \dot p_k \dot p_r \lproduct*{
  (\del_{p_k}\pair)^{\perp}, (\del_{p_r}\pair)^{\perp}}_{\fieldSp}\\
  &= \half \dot p_k \dot p_r g_{p_kp_r}.
\label{eq:gl-kin-energy-moduli}
\end{align}

The coefficients $g_{p_kp_r}$ determine a metric in moduli
space. Manton proposed an interpretation of
\eqref{eq:gl-kin-energy-moduli} in another context
\cite{manton_remark_1982}. In our language, the static energy in the
sub-bundle $\fieldSp'$ must be preserved by solutions of the
Bogomonly's equations, because they are energy minimisers. Thence,
$\Energy[\dot\pair]$ approximates the energy of slow moving solutions
of the full field equations, corresponding to the Ginzburg-Landau
functional dependent in time, not the one considered here. Equation
\eqref{eq:gl-kin-energy-moduli} opens the possibility to study the
dynamics of the full field equations, at some order of
approximation in the low energy regime. It was Samol's who proved that
this metric depends only in the first derivatives of $\hf$ at the set
of zeros \cite{samols1992}, thus obtaining a localisation
formula for moduli space. For non-coalescent vortices, i.e. if each of
the zeros of the Higgs field is simple, letting,

\begin{equation}
\label{eq:h-def}
b_k(p_1, \ldots, p_n) = 2 \eval{\conj\del}{x = p_k} \left( \log\abs\hf^2
  - \log \abs {x - p_k}^2 \right),  
\end{equation}

then the metric coefficients in complex coordinates are,

\begin{equation}
\label{eq:samols-complex}
g_{k\conj{r}} = \delta_{kr} + 2 \pdv{p_k}[b_r].
\end{equation}

Samols' metric is remarkable, because it shows how the energy of a
field configuration depends on local data and converts a
problem in field theory into a problem on Riemannian geometry. Samol's
metric is not only Riemannian, it is also Kähler geometry, as was also
proved by him. We should also remark that even if moduli space is ill
defined, for example, if $\lambda \neq 1$ there are no
Bogomolny's equations and therefore \eqref{eq:samols-complex} is not
valid, the geometry of orthogonal projections in $\fieldSp'$ is still
valid. 




%%% Local Variables:
%%% TeX-master: "../../../geometric-models.tex"
%%% End:


==> chapters/vav-euclidean/sections/not-needed-anymore.tex <==
Now we consider the linearization of the regularised Taubes'
equation. Recall  
$\fnth_\epsilon$ depends smoothly on core positions. The derivatives 
$d\fnth_\epsilon$ and $\del_\epsilon\fnth_\epsilon$ are solutions to
two related  
linear elliptic equations,
%
\begin{align*}
    -\laplacian\,d\fnth_\epsilon &= \fnVmu(\fnv_\epsilon + \fnth_\epsilon)\,
    d\fnth_\epsilon 
    + \fnVmu(\fnv_\epsilon + \fnth_\epsilon)\,d\fnv_\epsilon
    + d\fng_\epsilon,\\
    -\laplacian\,\del_\epsilon\fnth_\epsilon 
    &= \fnVmu(\fnv_\epsilon + \fnth_\epsilon)\,
    \del_\epsilon\fnth_\epsilon 
    + \fnVmu(\fnv_\epsilon + \fnth_\epsilon)\,\del_\epsilon\fnv_\epsilon
    + \del_\epsilon\fng_\epsilon.
\end{align*}

Let 
%
\begin{align*}
  a_\epsilon = \fnVmu(\fnv_\epsilon + \fnth_\epsilon), &&
  b_\epsilon = a_\epsilon\,d\fnv_\epsilon + d\fng_\epsilon, &&
  b'_\epsilon = a_\epsilon\,\del_\epsilon\fnv_\epsilon + \del_\epsilon\fng_\epsilon,
\end{align*}

\begin{lemma}
The functions $a_\epsilon$, $d\fng_\epsilon$, $\del_\epsilon\fng_\epsilon$ 
have the limits,
%
\begin{gather*}
\lim_{\epsilon \to 0} \norm*{a_\epsilon - \frac{2}{\cmu + 
1}}_{\spL^p} = 0, \qquad p > 2/3,\\[6pt]
\lim_{\epsilon \to 0}\,\norm{d\fng_\epsilon}_{\spL^p}
= \lim_{\epsilon \to 0}\,\norm{\del_\epsilon\fng_\epsilon}_{\spL^p}
= 0, \qquad p > 2/5.
\end{gather*}
\end{lemma}

\begin{proof}
$a_\epsilon \to \frac{2}{\cmu + 1}$ as $\epsilon \to 0$ pointwise. 
Let $R > 0$, $\Omega = \plane \setminus \disk_R(0)$, the
proof of proposition \ref{prop:vav-euc-fnth-unif-conv} shows that 
 $v_\epsilon \to 0$ uniformly in $\plane\setminus\disk_R(0)$; by this
  result and the uniform 
 convergence of $\fnth_\epsilon$ we have 
 $a_\epsilon \to \frac{2}{\cmu + 1}$ 
 uniformly as $\epsilon\to 0$ outside a local region containing the 
 origin. Let 
 $t_\epsilon(x) = \fnv_\epsilon(x) + \fnth_\epsilon(x)$, a straightforward 
 calculation shows,
 %
 \begin{align*}
     \abs*{a_\epsilon - \frac{2}{\cmu + 1}} &= 
     \frac{2}{\cmu + 1}
     \abs*{\frac{(\cmu^2e^{t_\epsilon} - 1)
     \,(e^{t_\epsilon} - 1)}{(\cmu\,e^{t_\epsilon} + 1)^2}},
 \end{align*}
 %
 the right side of this equation is a continuous function in 
 $\plane\setminus\set{\pm\epsilon}$ with removable singularities at the cores. Assume $\epsilon < R$, so that if $\abs{x} > R$,
 %
 \begin{align*}
     \abs{x} - R < \abs{x} - \epsilon \leq \abs{x \pm \epsilon}.
 \end{align*}
 
 As $\abs{x} \to \infty$ we have the asymptotic estimate,
 %
 \begin{align*}
    \abs*{a_\epsilon - \frac{2}{\cmu + 1}} 
    &\leq  
    \frac{2C}{\cmu + 1}
    \abs{e^{t_\epsilon} - 1}\\
    &\leq C\,\abs{t_\epsilon}\\
    &= \frac{C\epsilon\,\abs{x_1}}{
    \abs{x - \epsilon}^2\abs{x + \epsilon}^2}\\
    &\leq \frac{
    C\epsilon\abs{x_1}}{(\abs{x} - R)^4}.
 \end{align*}
 
 Therefore, if $p > 2/3$
 %
 \begin{align*}
     \norm*{a_\epsilon - \frac{2}{\cmu + 1}}_{\spL^p(\Omega)} 
     \leq C\,\epsilon\,\norm*{
     \frac{\abs{x_1}}{
     (\abs{x} - R)^4}}_{\spL^p(\Omega)} \to 0,
 \end{align*}
 %
 as $\epsilon \to 0$. On the other hand, $\fnVmu$ is bounded, implying the 
 existence of a
 constant $C$ such that,
 %
 \begin{align*}
    \int_{\disk_R(0)} \abs*{a_\epsilon - \frac{2}{\cmu + 1}}^p\,dx
    < C,
 \end{align*}
%
by the dominated convergence theorem,
%
 \begin{align*}
    \lim_{\epsilon \to 0}
    \int_{\disk_R(0)} \abs*{a_\epsilon - \frac{2}{\cmu + 1}}^p\,dx = 0,
 \end{align*}
 %
 hence, $a_\epsilon \to \frac{2}{\cmu + 1}$ in $\spL^p$ for any $p > 2/3$. 
 
 To compute the norm of $dg_\epsilon$, note that 
  %
  \begin{align*}
      g'(t) = \frac{-16\,t}{(1 + t^2)^3},
  \end{align*}
  %
  hence,
  %
  \begin{align*}
      \del_i g_\epsilon = 
      g'(\abs{x - \epsilon}) \, \frac{
      (x_j - \epsilon\delta_{1j})}{
      \abs{x - \epsilon}}
      - g'(\abs{x + \epsilon}) \, \frac{
      (x_j + \epsilon\delta_{1j})}{
      \abs{x + \epsilon}}
  \end{align*}
 %
 has removable singularities at $\pm\epsilon$ and 
 converges pointwise to 0 as $\epsilon \to 0$. Let us assume 
  $p > 2/5$, if $\epsilon < R$, we have the bound,
 %
 \begin{align*}
     \norm{\del_ig_\epsilon}_{\spL^p(\Omega)} \leq  
     C \norm*{
     \frac{\abs{x} + R}{
     (1 + (\abs{x} - R)^2)^3}
     }_{\spL^p(\Omega))} < \infty.
 \end{align*}
 
 Likewise, $\del_i g_\epsilon$ is also bounded in $\spL^p(\disk_R(0))$,
  the bound being given by any constant $C > 64 R$. By the dominated
  convergence theorem,
 %
 \begin{align*}
     \lim_{\epsilon\to 0}\,\norm{\del_ig_\epsilon}_{\spL^p} = 0.
 \end{align*}
 
 For $\del_\epsilon\fng_\epsilon$ the proof is the same, because,
 %
 \begin{align*}
    \del_\epsilon g_\epsilon = 
      -g'(\abs{x - \epsilon}) \, \frac{
      x_1 - \epsilon}{
      \abs{x - \epsilon}}
      - g'(\abs{x + \epsilon}) \, \frac{
      x_1 + \epsilon}{
      \abs{x + \epsilon}}
 \end{align*}
 %
 has the same removable singularities and order of convergence at 
 infinity.
 \end{proof}
 
 \begin{lemma}
 Let $R > 0$, $\Omega = \plane\setminus \disk_R(0)$ and $p > \half$, 
 we have the following convergences,
 %
 \begin{gather*}
 \lim_{\epsilon\to 0}\,
 \norm{a_\epsilon\del_i\fnv_\epsilon}_{\spL^p} 
 = 
 \lim_{\epsilon\to 0}\,
 \norm{a_\epsilon\del_\epsilon\fnv_\epsilon}_{\spL^p(\Omega)} 
 = 0.
 \end{gather*}
 \end{lemma}
 
 \begin{proof}
 Let 
 us compute $a_\epsilon\,dv_\epsilon$,
 %
 \begin{align*}
    a_\epsilon\,\del_iv_\epsilon &=
    2a_\epsilon \brk( 
    \frac{x_i - \epsilon\delta_{1i}}{(1 + \abs{x - \epsilon}^2)\abs{x - \epsilon}^2}
     - \frac{x_i + \epsilon\delta_{1i}}{(1 + \abs{x + \epsilon}^2)\abs{x + \epsilon}^2}
     ).
 \end{align*}
 
 This is a well defined continuous family of functions, because the factor 
 $e^{v_\epsilon}$ in $a_\epsilon$ cancels the poles at $x = \pm\epsilon$. 
  We have the limit $\lim_{\epsilon\to 0} a_\epsilon\del_iv_\epsilon = 0$ pointwise. Let us assume $\epsilon < R$, 
%
\begin{align*}
    a_\epsilon = \frac{
    2(\cmu + 1) (1 + \abs{x + \epsilon}^2) (1 + \abs{x - \epsilon}^2)
     \abs{x - \epsilon}^2\,\abs{x + \epsilon}^2\,e^{\fnth_\epsilon}}{
     \brk(
     \cmu\,e^{\fnth_\epsilon}(1 + \abs{x + \epsilon}^2)\abs{x - \epsilon}^2 
     + (1 + \abs{x - \epsilon}^2)\abs{x + \epsilon}^2)^2}.
\end{align*}

%%%%%CHECK THIS PLEASE! %%%%%%%%
The denominator is a continuous function of $x$ and $\epsilon$ which is never 0, 
we conclude that 
$a_\epsilon\del_i\fnv_\epsilon$ is uniformly bounded in $\disk_R(0)$. 
By the domninated convergence theorem,
%
\begin{align*}
\lim_{\epsilon\to 0}\,\norm{a_\epsilon\del_i\fnv_\epsilon}_{\spL^p(\disk_R(0))} = 0,
\qquad p > 0.
\end{align*}

On the other hand, if $\abs{x} > R$,
%
\begin{align*}
    \abs*{a_\epsilon\del_i\fnv_\epsilon} &\leq C 
    \abs*{
    \frac{\abs{x_i}\, \brk(\abs{x + \epsilon}^2 - \abs{x - \epsilon}^2)
    ( 1 + 
    \abs{x + \epsilon}^2 + \abs{x - \epsilon}^2)}{
    (1 + \abs{x + \epsilon}^2)(1 + \abs{x - \epsilon}^2)
    \abs{x + \epsilon}^2\abs{x - \epsilon}^2}
    }\\
    &\quad+ \epsilon\,\delta_{1i}\,C\brk(
    \frac{1}
    {(1 + \abs{x - \epsilon}^2)\abs{x - \epsilon}^2}
    + \frac{1}{
    {(1 + \abs{x + \epsilon}^2)\abs{x + \epsilon}^2}})\\
    &\leq \epsilon \abs{x_i}\,\abs{x_1}\,C \brk(
    \frac{1}{\brk(1 + \brk(\abs{x} - \half)^2)^2\brk(\abs x - \half)^4}
    + \frac{2}{\brk(1 + \brk(\abs{x} - \half)^2)^2\brk(\abs x - \half)^2})\\
    &\quad+ \frac{2\epsilon\,\delta_{1i}\,C}{
    \brk(1 + \brk(\abs{x} - \half)^2)\brk(\abs x - \half)^2}.
\end{align*}

The right side of this inequality is converging to 0 in 
$\spL^p(\plane\setminus \disk_R(0))$ for $p > \half$. Therefore,
%
\begin{align*}
    \lim_{\epsilon\to 0}\,\norm{a_\epsilon\del_i\fnv_\epsilon}_{\spL^p(\plane)} = 0,
    \qquad p > \half.
\end{align*}

For $a_\epsilon\del_\epsilon\fnv_\epsilon$ we follow the same pattern, in this 
case we have, 
%
 \begin{align*}
    a_\epsilon\,\del_\epsilon\fnv_\epsilon &=
    -2\,a_\epsilon \brk( 
    \frac{x_1 - \epsilon}{(1 + \abs{x - \epsilon}^2)\abs{x - \epsilon}^2}
    + 
    \frac{x_1 + \epsilon}{(1 + \abs{x + \epsilon}^2)\abs{x + \epsilon}^2}
     ),
 \end{align*}
%
which converges pointwise to
%
\begin{align*}
 \frac{-8\,x_1}{(\cmu + 1)(1 + \abs{x}^2)\,\abs{x}^2}   
\end{align*}
%
 in the punctured plane $\plane\setminus\set{0}$. As for 
 $a_\epsilon\del_i\fnv_\epsilon$, each of these functions is in 
 $\spL^p$ for $p > 2/3$, however, the functions 
 %
 \begin{align*}
     \norm{a_\epsilon\del_i\fnv_\epsilon}_{\spL^p},
 \end{align*}
 %
 are divergent as $\epsilon \to 0$. 
\end{proof}


\begin{proposition}
There are constants $C > 0$ and $\epsilon_0$ such that,
%
\begin{align*}
\norm{d\fnth_\epsilon}_{\spL^2} \leq 
    C\,\norm{b_\epsilon}_{\spL^2}, &&
    \norm{\del_\epsilon \fnth_\epsilon}_{\spL^2} \leq 
    C\,\norm{b'_\epsilon}_{\spL^2}, 
\end{align*}
%
for all $\epsilon < \epsilon_0$. 
\end{proposition}

\begin{proof}
$2 (\cmu + 1)^{-1}$ is the common supremum of all the functions
$a_\epsilon$. Let $M$ be any common strict upper bound 
for all $a_\epsilon$ and let 
$\domain$ be a convex neighbourhood of the origin of  diameter 
$d < \pi/M$ as in the previous Lemma. Let $\delta > 0$ be a small 
positive number, by the 
dominated convergence theorem, there is $\epsilon_0 > 0$, such that 
if $\epsilon < \epsilon_0$,
%
\begin{gather*}
    \alpha_1 = \frac{2}{\cmu + 1} - \delta 
    < \frac{\int_\domain a_\epsilon\,\vol}{\vol(\domain)}, \\
    \alpha_2 = \frac{2}{\cmu + 1}\,
    \brk (1 - \frac{2}{M(\cmu + 1)}) -\delta 
    < \frac{1}{\vol(\domain)}\int_\domain a_\epsilon 
    \brk (1 - \frac{a_\epsilon}{M})\,\vol.
\end{gather*}

If $C > 0$ is such that,
%
\begin{align*}
\frac{1}{C} < \min \brk(m, 1, \alpha_1, 
    \frac{1 - \frac{M\,d}{\pi}}{1 + Cp(\domain)}, 
    \alpha_2),
\end{align*}
%
then by lemma~\ref{lem:vav-euc-coerc-cnst}, $1/C$ is a common
coercivity constant for the operators,
%
\begin{align*}
    B_\epsilon: \spH^1\times\spH^1 \to \reals, &&
    B_\epsilon(u, v) = 
    \lproduct{du, dv}_{\spL^2} + \lproduct{u,\,a_\epsilon v}_{\spL^2}.
\end{align*}

By elliptic regularity, $d\fnth_\epsilon$,  $\del_\epsilon\fnth_\epsilon$
are strong $\spH^2$ solutions to the problems.  
%
\begin{align*}
    -\laplacian d\fnth_\epsilon = a_\epsilon\,d\fnth_\epsilon 
    + b_\epsilon, &&
    -\laplacian \del_\epsilon\fnth_\epsilon 
    = a_\epsilon\del_\epsilon\fnth_\epsilon 
    + b'_\epsilon.
\end{align*}

Since the solutions are strong, we can apply integration 
by parts and coercivity to obtain the bound
%
\begin{align*}
    \frac{1}{C}\,\norm{d\fnth_\epsilon}_{\spH^1}^2 
    \leq 
    B_\epsilon(d\fnth_\epsilon, d\fnth_\epsilon)
    = \lproduct{-b_\epsilon, d\fnth_\epsilon}
    \leq \norm{b_\epsilon}_{\spL^2}\,\norm{d\fnth_\epsilon}_{\spL^2}.
\end{align*}

Hence,
%
\begin{align*}
    \norm{d\fnth_\epsilon}_{\spL^2} \leq 
    C\,\norm{b_\epsilon}_{\spL^2}.
\end{align*}

Analogously for $\del_\epsilon\fnth_\epsilon$.
\end{proof}



==> chapters/vav-sphere/commands.tex <==
% Utils
\newcommand*\vp{\mathbf{p}}
\newcommand*\vq{\mathbf{q}}

\DeclareDocumentCommand\brk{d()}{
  \left( #1 \right)
}

\newcommand*\surface{\Sigma}%

\DeclareMathOperator\potentialE{V}%

\newcommand*\hf{\phi}%
\newcommand*\gp{a}%
\newcommand*\del{\partial}%
\newcommand*\sphere{{\mathbb{S}^2}}%
\newcommand*\Diff{\mathcal{D}}%
\newcommand*\conj[1]{\overline{#1}}%
\newcommand*\half{\frac{1}{2}}%
\newcommand*\pbundle{P}%
\newcommand*\fbundle{F}%
\newcommand*\north{n}%
\newcommand*\pconnection{A}%
\newcommand*\pcurvature{F}%
\newcommand*\isometry{\mathcal{I}}
%\newcommand*\abs[1]{\lvert{#1}\rvert}%

\NewDocumentCommand\abs{sm}{
  \IfBooleanTF#1{
    \left\lvert{#2}\right\rvert
  }{
    \lvert{#2}\rvert
  }
}

% \NewDocumentCommand\set{sm}{
%   \IfBooleanTF#1{
%     \left\{ #2 \right\}
%   }{
%     \{ #2 \}
%   }
% }


\newcommand*\laplacian{\Delta}%

\newcommand*\vset{\mathcal{P}}%

\newcommand*\avset{\mathcal{Q}}%

\newcommand*\moduli{\mathcal{M}}%

\newcommand*\eval[2]{\left.{#1}\right\rvert _{#2}}%

\newcommand*\cf{\Omega}
\newcommand*\R{\mathbb{R}}%
\renewcommand*\C{\mathbb{C}}%
\newcommand*\pSpace{\mathbb{P}}%

\DeclareMathOperator\Jop{J}%

\DeclareMathOperator\Vol{Vol}%

\DeclareMathOperator\Energy{E}

\newcommand*\order{\mathcal{O}}%

\newcommand*\ldv{\mathcal{L}}%
\newcommand*{\moduliMetric}{g}
\newcommand*{\dv}[1]{\frac{d}{d{#1}}}

\newcommand*\Lp[2][2]{\mathrm{L}^{#1}(#2)}

\DeclareDocumentCommand{\pdv}{m g}
{
  \IfValueTF{#2}
  {
    \frac{\del #1}{\del #2}
  }
  {
    \frac{\del }{\del #1}	
  }
}


%%%% Analysis
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}

\newcommand*\dd{d}
\newcommand*\length{\ell}
\newcommand*{\disk}{\mathbb{D}}
\newcommand*{\htilde}{\tilde{h}}
\newcommand*{\hstar}{h^*}
\newcommand*{\ctilde}{\tilde{c}}
\newcommand*\cstar{c^*}
\newcommand*{\hhat}{\hat{h}}
\newcommand*{\plane}{\R^2}
\newcommand*{\Fstable}{\mathcal{F}}
\newcommand*{\feps}{f_\epsilon}
\newcommand*\Csp[2][0]{\mathrm{C}^{#1}(#2)}
\newcommand*{\Hsp}[2][1]{\mathrm{H}^{#1}(#2)}
\newcommand*{\Lsp}[2][2]{\mathrm{L}^#1(#2)}
\newcommand*{\Xsp}{\mathcal{X}}
%\newcommand*\norm[1]{\lvert\lvert#1\rvert\rvert}

\newcommand\dist{\mathrm{dist}}


\NewDocumentCommand\norm{sm}{
  \IfBooleanTF#1{
    \left\lvert\left\lvert#2\right\rvert\right\rvert
  }{
    \lvert\lvert#2\rvert\rvert
  }
}

\NewDocumentCommand\lproduct{sm}{
  \IfBooleanTF{#1}
  {\left\langle #2 \right\rangle}
  {\langle #2 \rangle}
}

\newcommand*{\Hnorm}[3][1]{\norm{#2}_{\Hsp[#1]{#3}}}

\newcommand*\wto\rightharpoonup\WithSuffix\newcommand\Hnorm*[3][1]{\norm*{#2}_{\Hsp[#1]{#3}}} 
\newcommand*{\Lnorm}[3][2]{\norm{#2}_{\Lsp[#1]{#3}}}
\WithSuffix\newcommand\Lnorm*[3][2]{\norm{#2}_{\Lsp[#1]{#3}}}
\newcommand*{\Lprod}[2][\sphere]{\langle #2 \rangle_{#1}}

\newcommand*{\set}[1]{\left\{#1\right\}}
\WithSuffix\newcommand\set*[1]{\{#1\}}

\newcommand*{\vd}[1]{
  \IfEqCase{#1}{
    {1}{v'}
    {2}{v''}
  }[\PackageError{V}{Only 1 or 2 allowed as options, got #1}{}]
}

\newcommand*\uniformlyto\rightrightarrows
\newcommand*\htildeEps{\htilde^\epsilon}
\newcommand*\ctildeEps{\ctilde^\epsilon}
\newcommand*\vdeps[1]{{\vd{#1}}^\epsilon}
\newcommand*\grad{\nabla}
\newcommand*\delEps{\del_\epsilon}
\newcommand*\proj{\mathbb{P}}


%Linear section commands
\newcommand*\ueps{u}
\newcommand*\afn{a}
\newcommand*\bfn{b}
\newcommand*\manifold{M}
\newcommand*\metric[1]{\langle{#1}\rangle}
\newcommand*\aForm{\mathcal{A}}
% \newcommand*\fFunc{\mathcal{F}}
\newcommand*\fFunc{B}
\newcommand*\hSp{\mathcal{H}}
\newcommand*\uBound{K_1}
\newcommand*\cBound{K_2}
\newcommand*\vol{\mathrm{Vol}}
\newcommand*\suchthat{\;\middle\vert\;}
\newcommand*\intManifold{\int_{\manifold}}
\newcommand*\vortexSet{\mathcal{P}}
\newcommand*\avortexSet{\mathcal{Q}}
\newcommand*\vavSet{\mathcal{S}}
\newcommand*\Dfrechet{\mathcal{D}}

%%%%%%%%%%%

\newcommand*\brackets{}

%%%%%%%%%%%

% Spaces

\newcommand*\domain{\mathscr{D}}

%\DeclareMathOperator\Lsp{L}
%\DeclareMathOperator\Hsp{H}

%\newcommand*\lsp[1]{\Lsp^{#1}}
%\newcommand*\hsp[1]{\Hsp^{#1}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "master"
%%% End:


==> chapters/vav-sphere/sections/elliptic-problem-sphere.tex <==
\newcommand*{\delEps}{\del_{\epsilon}}
\newcommand*{\cstar}{c_{*}}
\newcommand*{\uniformlyto}{\rightrightarrows}
\newcommand*{\hstar}{h_{*}}
\newcommand*{\htildeEps}{\tilde h_{\epsilon}}
\newcommand*{\ctildeEps}{\tilde c_{\epsilon}}
\newcommand*{\dd}{d}
\newcommand*{\Csp}{\mathrm{C}^{0}}


We are interested in describing the
behaviour of solutions to the equation

\begin{equation}
  \label{eq:v-av}
  -\laplacian_{\sphere} u = \Fstable(u) + 4\pi(\delta_p - \delta_q),
\end{equation}
%
Equation \eqref{eq:v-av} is the \emph{vortex-antivortex}
equation. $\sphere$ denotes the round sphere of radius $R$. We can assume in a stereographic chart the point $p$ is located at
position $\epsilon$ and $q$ is at position $-\epsilon$, $0 < \epsilon
\leq 1$, in this projective chart,
%
% to determine the volume of moduli space  it is necessary to
% compute the limit 


% \begin{equation}
%   \label{eq:moduli-limits}
%   \lim_{\epsilon \to 0} \epsilon b_\epsilon(\epsilon,-\epsilon), 
% \end{equation}

% here, the sub index $b_{\epsilon}$ is to emphasise the dependence of
% the coefficient $b_1$ in the position of the pair. 

\begin{equation}
  \label{eq:v-coords-ster}
  v = \log\abs{z - \epsilon}^2 - \log\abs{z + \epsilon}^2.
\end{equation}

In this section we will determine bounds for  $h$,  $\delEps h$ and some of its derivatives, where $h$ is the solution to equation \eqref{eq:regular-taubes-bps} in this context. We will use $\epsilon$ as super-index to stress the dependence of the problem in  pair separation. Now we prove two technical lemmas

\begin{lemma}\label{lem:mueps-delta-conv}
  Let $\mu_{\epsilon} = \pi^{-1}\epsilon^2(\epsilon^2 +
  \abs{w}^2)^{-2}d^2w$, then $\mu_{\epsilon} \to \delta_0$ in the
  following sense: if $\varphi$ is a measurable function in $\plane$
  such that $\lim_{\abs{w} \to 0} \varphi = L$ is finite and such that
  for any $R > 0$, $\abs{w}^{-4}\cdot\varphi
  \in \Lsp^1({\abs{w} \geq R})$, then

  
  \begin{equation}
    \lim_{\epsilon\to 0} \abs*{\int_{\plane}\varphi \mu_{\epsilon} - L}
    = 0.
    \label{eq:mueps-delta-conv}
  \end{equation}
\end{lemma}

\begin{proof}
  Let $\delta > 0$, and let $R > 0$ be such that if $0 < \abs{w} \leq
  R$, then
  \begin{equation}
    \label{eq:phi-lim}
    \abs{\varphi(w) - L} < \frac{
      \delta
    }{
      2
    }.
  \end{equation}

  Let $C = \int_{\abs{w} \geq R}\abs{w}^{-4}\abs{\varphi}$, since each
  $\mu_{\epsilon}$ is 
  a probability measure,

  \begin{align}
    \nonumber
    \abs*{
      \int_{\plane}\varphi\mu_{\epsilon} - L}
    &=
    \abs*{
      \int_{\plane} (\varphi - L) \mu_{\epsilon}
      }\\
    \nonumber
    &\leq
    \int_{\abs{w} \geq R} \abs{\varphi - L}\mu_{\epsilon}
    +
      \int_{\abs{w} \leq R} \abs{\varphi - L}\mu_{\epsilon}\\
    \nonumber
    &\leq
      \left(
      \frac{
      C
      }{
      \pi
      }
      +
      \frac{
       \pi\abs{L}
      }{
      R^2
      }
      \right)
      \epsilon^2
      +
      \frac{
      \delta\cdot R^2
      }{
      2\left(\epsilon^2 + R^2\right)
      }\\
    \label{eq:measure-bound}
    &\leq
      \left(
      \frac{
      C
      }{
      \pi
      }
      +
      \frac{
       \pi\abs{L}
      }{
      R^2
      }
      \right)
      \epsilon^2
            +
      \frac{
      \delta
      }{
      2
      }.
  \end{align}

  Hence there is a constant $K > 0$ such that if $\epsilon < K$, then

  \begin{equation}
    \label{eq:eps-delta-measure}
    \abs*{
      \int_{\plane}\varphi\mu_{\epsilon} - L} \leq \delta.
  \end{equation}

\end{proof}

Lemma~\ref{lem:mueps-delta-conv} can be explained intuitively noting
that the family of functions 
%
\begin{equation}
  \label{eq:feps-to-delta}
  f_{\epsilon}(w) = \frac{\epsilon^2}{\left(\epsilon^2 + \abs{w}^2\right)^2}
\end{equation}
%
is converging in measure to a Dirac delta function $\delta(w)$. 
%as
% can be seen in figure~\ref{fig:feps-to-delta}. 

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=.5\textwidth]{img/eps-conv-delta.pdf}
%   \caption{A sample of the family $f_\epsilon(w)$.}
%   \label{fig:feps-to-delta}
% \end{figure}

\par

\input{chapters/vav-sphere/sections/linearised-problem-lemma.tex}  
  
With these two lemmas, we move forward to find uniform bounds for $h^\epsilon$ and its derivatives. Let $c^*$ be the only solution to the equation
%
\begin{equation*}
    \Fstable_0(c^*) = 0,
\end{equation*}
%
we will prove that $h^\epsilon$ converges strongly to $c^*$ in $\Hsp^2(\sphere)$ as $\epsilon \to 0$ adapting an argument found in \cite{tarantello1996multiple}. From this convergence and Sobolev's embedding we will also have that $h^\epsilon \to c^*$ uniformly as $\epsilon\to 0$. Since $\Fstable_0$ is a bounded function, the functions $-\laplacian_{\sphere} h^\epsilon$ are uniformly bounded in $\Lsp^2({\sphere})$. Let,
%
\begin{align*}
    \ctildeEps &= \frac{1}{4\pi R^2}\int_\sphere  h^\epsilon \star 1, &
    \htildeEps &= h^\epsilon - \ctildeEps,
\end{align*}
%
then $-\laplacian_\sphere \htildeEps$ is also uniformly bounded in $\Lsp^2({\sphere})$. By the elliptic estimate, there is a constant 
$C$, such that 

\begin{equation}
  \label{eq:htilde-bounde-hsp2}
  \norm{\htildeEps}_{\Hsp^2(\sphere)} \leq C, \qquad \forall\epsilon.
\end{equation}

%%%Todo esto va a cambiar
% Note that the function $\epsilon \mapsto \ctildeEps$ is bounded, because otherwise, there is a sequence $\epsilon_n$ for which 
% since the function $c^\epsilon$ is bounded, after passing to a
% subsequence if necessary we can assume $\ctilde_n \to c'$ for some $c'$. 
%%%

By Sobolev's embedding, the family $\htildeEps$ is also uniformly bounded in $\Csp{\sphere}$.  We prove that $\lim_{\epsilon \to 0} \norm{h^\epsilon - c^*}_{\Hsp^2(\sphere)} = 0$ by showing that for any sequence $\epsilon_n \to 0$, the sequence $h_n = h^{\epsilon_n}$ has a subsequence converging to $c^*$ in $\Hsp^2(\sphere)$. Let $\ctilde_n = \ctilde^{\epsilon_n}$ and  $\htilde_n = \htilde^{\epsilon_n}$, by Alouglu's theorem we can assume $\htilde_n \wto \hstar$ in
$\Hsp^1(\sphere)$ for some $h^*\in \Hsp^1(\sphere)$. By Rellich's theorem, we can also assume the strong convergence $\htilde_n \to h^*$ in $\Lsp^2({\sphere})$. Let $v_n = v_{\epsilon_n} - v_{-\epsilon_n}$, we claim there is a convergent subsequence of $\ctilde_n$. Assume towards a contradiction this is false, then there is a subsequence $c_{n_k}$ diverging to $\pm\infty$. Suppose $c_{n_k} \to \infty$ and let $f_k = \Fstable_0(v_{n_k} + h_{n_k})$, by the divergence theorem,

\begin{equation*}
    \int_{\sphere} f_k \star 1 
    = \int_{\sphere} \laplacian_{\sphere} h_{n_k} *1 = 0.
\end{equation*}

Since $v_{n_k} \to 0$ pointwise whereas $\htilde_{n_k}$ is uniformly bounded, $f_k \to 2(1 - \tau)$ pointwise, while $\abs {f_k}$ is uniformly bounded. By the dominated convergence theorem,
%
\begin{equation*}
    \lim \int_{\sphere} f_k *1 = 8\pi R^2 (1 - \tau),
\end{equation*}
%
which is a contradiction. If $c_{n_k} \to -\infty$ an similar claim holds. After passing to a subsequence if necessary, we can assume the convergence $c_n \to c'$ from which we have $h_n \to  c' + \hstar$ in $\Lsp^2(\sphere)$. Applying the mean value theorem,

\begin{equation}
  \label{eq:a-priori-estimate}
  \abs{\Fstable_0\pbrk{v_n + h_n} -
    \Fstable_0\left(c' + \hstar\right)} \leq 2\abs{
      v_n + h_n - c' - \hstar
  }.
\end{equation}

Let $\varphi \in \Hsp^1(\sphere)$, then

\begin{multline} \label{eq:1}
  \abs*{
    \int_{\sphere} \left(
      \Fstable_0(v_n + h_n) -
      \Fstable_0(c' + \hstar)
    \right)\,\varphi \star 1
  }
  \leq 
  2 \int_{\sphere} \abs{
      v_n + h_n - c' - \hstar
    }\abs{
      \varphi
    } \star 1\\
    \leq 2 \pbrk{
      \norm{v_n}_{\Lsp^2(\sphere)} +
      \norm{h_n - c' - \hstar}_{\Lsp^2(\sphere)}
    }
     \norm{\varphi}_{\Lsp^2(\sphere)}. 
\end{multline}

Note that $\norm{v_n}_{\Lsp^2(\sphere)} \to 0$, because if we change variables $z \mapsto \epsilon w^{-1}$ and apply lemma~\ref{lem:mueps-delta-conv},

\begin{equation}
\norm{v_n}_{\Lsp^2(\sphere)}^2 = \int_{\plane}
  \log^2\left(
    \frac{
      \abs{w - 1}^2
    }{
      \abs{w + 1}^2
    }
    \right) \frac{
      \epsilon_n^2d^2w
    }{
      \pbrk{\epsilon_n^2 + \abs{w}^2}^2
    } \to 0.
  \end{equation}

Then from equation (\ref{eq:1}), 

\begin{equation}
  \Fstable_0 \left( v_n + h_n \right) \wto\Fstable_0\left(c' + \hstar\right), \qquad
  \text{in } \Lsp^2(\sphere).
  \label{eq:w-fstable-convergence}
\end{equation}

On the other hand, $\laplacian_{\sphere} h_n$
converges also to $\laplacian_{\sphere} (c' + \hstar)$ in the weak
sense, and we infer from equation \eqref{eq:1} that $c' + \hstar$ is a weak
solution to the equation,

\begin{equation}
  \label{eq:weak-star-convergence}
  -\laplacian_{\sphere}(c' + \hstar) = \Fstable_0(c' + \hstar).
\end{equation}

A bootstrap argument shows $c' + \hstar$ is a smooth
function, but recall that $\Fstable_0$ is an increasing function, then from the maximum principle, $c' +
\hstar$ can only be a solution to \eqref{eq:weak-star-convergence} if
$\hstar \equiv 0$ and $\Fstable_0(c') = 0$. Monotony of $\Fstable_0$ then implies $c' = c^*$. Therefore, $h_n \to c^*$ strongly in $\Lsp^2({\sphere})$. On the other hand, by the mean value theorem,
%
% if we take $\varphi = h_n - \cstar$, and substitute into
% \eqref{eq:1}, we have,

% \begin{equation}
%   \label{eq:grad-htilde-eps-bound}
%   \norm{\grad(h_n - \cstar)}^2_{\Lsp\sphere} \leq
%   2 \left(
%     \norm{v_n}_{\Lsp\sphere}
%   +
%       \norm{
%         h_n - \cstar
%       }_{\Lsp\sphere}
%   \right)
%      \norm{h_n - \cstar}_{\Lsp\sphere} \to 0,
% \end{equation}

% hence $h_n \to \cstar$ strongly in $\Hsp\sphere$. 
%
% We can also infer from 
% equation~\eqref{eq:grad-htilde-eps-bound} and Poincar\'e's inequality
% the limit  $\lim_{\epsilon\to 0} \norm{\htildeEps}_{\Lsp\sphere} =
% 0$. 

\begin{multline}
  \norm{\laplacian_{\sphere}
  h_n}^2_{\Lsp^2(\sphere)} 
  = \int_{\sphere}F(v_n 
  + h_n)^2 \star 1
  = \int_{\sphere} F'(\xi)^2(v_n +
   h_n - \cstar)^2 \star 1 \\
  \leq 4\left( \norm{v_n}^2_{\Lsp^2(\sphere)}
  + \norm{h_n - c^*}^2_{\Lsp^2(\sphere)}\right) \to 0.
\end{multline}

Hence, $\norm{\htilde_n}_{\Hsp^2(\sphere)} 
\to 0$ by the elliptic estimate which on the other hand implies $\norm{h_n - c^*}_{\Hsp^2(\sphere)} 
\to 0$. Therefore, $\lim_{\epsilon\to 0} h^{\epsilon} = c^*$ in
$\Hsp^2(\sphere)$ and by Sobolev's embedding  
$h^{\epsilon}\uniformlyto c^*$. Uniform
convergence implies the
existence of positive constants $C_1$, $C_2$ such that

\begin{equation}
  \label{eq:uniform-conv-boundedness}
  \frac{
    8 e^{h^\epsilon}
  }{
    \left(\abs{z - \epsilon}^2e^{h^\epsilon} + \abs{z + \epsilon}^2\right)^2
  } \leq \frac{
    C_1
  }{
    \left(\abs{z - \epsilon}^2 C_2 + \abs{z + \epsilon}^2\right)^2
  }.
\end{equation}

We will use \eqref{eq:uniform-conv-boundedness} and the elliptic
estimates to show the family $\dd{h^{\epsilon}}$ is uniformly bounded. Let us denote $v^{\epsilon} + h^\epsilon$ by $t^{\epsilon}$, if we denote coordinates in $\sphere$ in south pole stereographic projection as $z = x + yi$, a straightforward computation shows 

\begin{equation}
  \label{eq:fstable-derivative}
  \begin{aligned}
  \del_x(\Fstable_0(t^{\epsilon}))
  &= \Fstable_0'(t^{\epsilon}) \left(
  \frac{
    2(x (\abs{z + \epsilon}^2 - \abs{z - \epsilon}^2) - \epsilon
    (\abs{z + \epsilon}^2 + \abs{z - \epsilon}^2))
  }{ \abs{z - \epsilon}^2 \abs{z + \epsilon}^2}
  + \del_x h^{\epsilon}
  \right),\\
  \del_y(\Fstable_0(t^{\epsilon}))
  &= \Fstable_0'(t^{\epsilon}) \left(
  \frac{
    2 y (\abs{z + \epsilon}^2 - \abs{z - \epsilon}^2)
  }{ \abs{z - \epsilon}^2 \abs{z + \epsilon}^2}
  + \del_y h^{\epsilon}
  \right).
  \end{aligned}
\end{equation}

On the other hand,

\begin{equation}
  \label{eq:fStabledash-teps}
  \begin{gathered}
  \Fstable_0'(t^{\epsilon}) = \frac{
    8 e^{h^{\epsilon}}
    \abs{z - \epsilon}^2\abs{z + \epsilon}^2
  }{
    \left(\abs{z - \epsilon}^2e^{h^{\epsilon}} + \abs{z + \epsilon}^2\right)^2
  },\\
      \abs{
      \abs{z + \epsilon}^2 - \abs{z - \epsilon}^2
    } \leq
    4 \epsilon\abs{z},\\
    \abs{z + \epsilon}^2 + \abs{z - \epsilon}^2 \leq
    2\,(\abs{z}^2 + \epsilon^2).
  \end{gathered}
\end{equation}

By equations \eqref{eq:uniform-conv-boundedness},
\eqref{eq:fstable-derivative}, \eqref{eq:fStabledash-teps},

\begin{equation}
  \label{eq:dFstable-estimate}
  \abs{d(\Fstable_0(t^{\epsilon}))}_{\plane} \leq 2
  C_1 \frac{
    8\epsilon \abs{z}^2 + 2 \epsilon (\abs{z}^2 +
    \epsilon^2)
  }{
    \left(\abs{z - \epsilon}^2C_2 + \abs{z + \epsilon}^2\right)^2
  } + 2\abs{d h^{\epsilon}}_{\plane},
\end{equation}

hence,

\begin{align}
  \norm{\laplacian_{\sphere}d h^{\epsilon}}_{\Lsp^2(\sphere)} &=
  \norm{d(\Fstable_0(t^{\epsilon}))}_{\Lsp^2(\sphere)} \nonumber\\ 
  &=
  \norm{d(\Fstable_0(t^{\epsilon}))}_{\Lsp^2(\plane)}\nonumber\\
  &\leq
  2C_1
  \norm*{
   \frac{
    10\epsilon\abs{z}^2
  }{
    \left(\abs{z - \epsilon}^2C_2 + \abs{z + \epsilon}^2\right)^2
  }
}_{\Lsp\plane}\nonumber\\
&\quad + 2C_1
\norm*{
  \frac{
    2\epsilon^3
  }{
    \left(\abs{z - \epsilon}^2C_2 + \abs{z + \epsilon}^2\right)^2
  }
}_{\Lsp^2(\plane)}\nonumber\\
&\quad + 2 \norm{d h^{\epsilon}}_{\Lsp^2(\plane)}.
\label{eq:laplacian-dheps-bound}
\end{align}

Let us denote the first two terms in the upper bound as $(I)$ and
$(II)$ respectively, if we change variables to $z \mapsto
\epsilon w$, we have,
%
\begin{align}
  \label{eq:norm-I-bound}
  (I)^2 &= \int_{\plane} \frac{
    10^2 \abs{w}^4d^2\omega
  }{
    \pbrk{
    \abs{w - 1}^2C_2 + \abs{w + 1}^2
    }^{4}
  },\\
  \label{eq:2-ad}
  (II)^2 &= \int_{\plane} \frac{
    4\,d^2\omega
  }{
    \pbrk{
    \abs{w - 1}^2C_2 + \abs{w + 1}^2
    }^{4}
  }.
\end{align}
%
\eqref{eq:norm-I-bound} and \eqref{eq:2-ad} are
convergent because for big $\abs{w}$, they are of order at least
$\abs{w}^{-4}$. Since $\norm{\dd h^{\epsilon}}_{\Lsp^2(\plane)} =
\norm{\dd h^{\epsilon}}_{\Lsp^2(\sphere)} \to
0$, by \eqref{eq:laplacian-dheps-bound} there exists an uniform bound
$C$ for
$\norm*{\laplacian_{\sphere}\dd h^{\epsilon}}_{\Lsp^2(\sphere)}$. Thence, 

\begin{equation}
  \label{eq:dhtilde-eps-bound}
  \norm{d h^{\epsilon}}_{\Csp(\sphere)} \leq
  C_1 \norm{d h^{\epsilon}}_{\Hsp^2(\sphere)} \leq C.
\end{equation}

\subsection{Uniform bound for $\epsilon\del_x^2 h^\epsilon$}

Having found a uniform bound for the family $d h^{\epsilon}$, we will 
estimate $\norm{\del_x^2 h^\epsilon}_{\Csp(\sphere)}$  and $\norm{\del_x\del_{\epsilon}\htildeEps}_{\Csp(\sphere)}$. Let us
start estimating the $\Csp\sphere$ norm of $\del^2_x h^\epsilon$. Firstly,

\begin{equation}
  \label{eq:linf-delx2-estimator}
  \norm*{\del^2_x h^\epsilon}_{\Csp(\sphere)} \leq
  C_1 \norm*{\del^2_x h^\epsilon}_{\Hsp^2(\sphere)} \leq
  C_2 \norm*{\laplacian_{\sphere}\del_x^2 h^\epsilon}_{\Lsp^2(\sphere)},
\end{equation}

for suitable constants $C_1$, $C_2$. After a straightforward calculation,

\begin{multline}
  \laplacian \del^2_x h^\epsilon =
  \del^2_x\left(\frac{
    \Fstable_0(t^{\epsilon})
  }{
    (1 + \abs{z}^2)^2 
  }\right) =
  \frac{
    24x^2 \Fstable_0(t^{\epsilon})
  }{
    (1 + \abs{z}^2)^4
  }
  - \frac{4\Fstable_0(t^{\epsilon})}{(1 + \abs{z}^2)^3} \\
  - \frac{
    8x\del_x(\Fstable_0(t^{\epsilon}))
  }{
    (1 + \abs{z}^2)^3
  }
  + \frac{
    \del^2_x (F_0(t^\epsilon))
  }{
    (1 + \abs{z}^2)^2
  }, 
\end{multline}

where the Laplacian operator without subindex is the euclidean Laplace's operator, $\del_x^2 + \del_y^2$. Hence,

\begin{equation}
  \label{eq:laplace-plane-del2x-htildeeps-bound}
  \norm*{\laplacian_{\sphere}\del^2_x h^\epsilon}_{\Lsp^2(\sphere)} \leq
  10 \norm{\Fstable_0(t^{\epsilon})}_{\Lsp^2(\sphere)} +
  16 \norm{d(\Fstable_0(t^{\epsilon}))}_{\Lsp^2(\sphere)} + 
  \norm*{\del^2_x(\Fstable_0(t^{\epsilon}))}_{\Lsp^2(\sphere)}.
\end{equation}

The first term on the right is bounded because $\Fstable_0$ is a bounded
function, the second term was proved bounded in equation
(\ref{eq:laplacian-dheps-bound}). Let us compute
$\del^2_x(\Fstable_0(t^{\epsilon}))$,
 
\begin{equation}
  \label{eq:del2-x-fstable}
  \del^2_x(\Fstable_0(t^{\epsilon})) =
  2\Fstable_0''
  (
  t^{\epsilon})\cdot \left(
    \del_xv^\epsilon +\del_x h^\epsilon\right)^2 + 2\Fstable_0'(t^{\epsilon})\cdot
    \left(
      \del^2_xv^\epsilon + \del^2_x h^\epsilon
    \right).
\end{equation}

The $\mathrm{L}^2$ norm of the first two terms in
\eqref{eq:del2-x-fstable} have already been shown bounded. We will
compute the remaining terms and estimate their norms.

\begin{align}
  \label{del2x-v1d-v2d}
  \del^2_xv^{\epsilon} = 2 \left(
  \frac{
    \abs{z - \epsilon}^2 - 2(x - \epsilon)^2
  }{
    \abs{z - \epsilon}^4
  }
  - \frac{
    \abs{z + \epsilon}^2 - 2 (x + \epsilon)^2
  }{
    \abs{z + \epsilon}^4
  }
  \right),
\end{align}

by equations \eqref{eq:fStabledash-teps} and \eqref{del2x-v1d-v2d},

\begin{equation}\label{eq:3-ad}
\abs*{\Fstable'(t^{\epsilon})\cdot\del^2_xv^{\epsilon}}_{\plane}
\leq
\frac{
  C_1(\abs{z - \epsilon}^2 + \abs{z + \epsilon}^2)
}{
 \left(
   \abs{z - \epsilon}^2C_2 + \abs{z + \epsilon}^2 
   \right)^2}.
% \frac{
%   C_1\abs{z - \epsilon}^2\abs{z + \epsilon}^2
% }{
%  \brackets(
%    \abs{z - \epsilon}^2C_2 + \abs{z + \epsilon}^2 
%  )^2}\cdot \abs{
% \frac{
%     \abs{z - \epsilon}^2 - 2(x - \epsilon)^2
%   }{
%     \abs{z - \epsilon}^4
%   }
%   - \frac{
%     \abs{z + \epsilon}^2 - 2 (x + \epsilon)^2
%   }{
%     \abs{z + \epsilon}^4
%   }
% }
\end{equation}

The bound in \eqref{eq:3-ad} decays as $\abs{z}^{-2}$ as $\abs{z} \to
\infty$, changing variables to $z \mapsto \epsilon w$, 

\begin{align}
 \nonumber
  \norm*{\Fstable'(t^{\epsilon})\cdot\del^2_xv^{\epsilon}}_{\Lsp^2(\sphere)}^2
  &\leq
  \int_{\plane}
  \frac{
  C_1^2(\abs{z - \epsilon}^2 + \abs{z + \epsilon}^2)^2
}{
 \left(
   \abs{z - \epsilon}^2C_2 + \abs{z + \epsilon}^2 
   \right)^4}\,
 d^2z
 \\
 \nonumber
 &= \frac{
   C_1^2
 }{
   \epsilon^2
 }
 \int_{\plane}
 \frac{
  (\abs{w - 1}^2 + \abs{w + 1}^2)^2
}{
 \left(
   \abs{w - 1}^2C_2 + \abs{w + 1}^2 
   \right)^4} d^2w\\
  \label{eq:4-ad}
 &= \frac{
   C
 }{
   \epsilon^2
 }.
\end{align}

We quote also $\Fstable_0''(t^{\epsilon})$ and $\del_xv^{\epsilon}$: 

\begin{equation}\label{eq:fdd-delx-vd}
  \begin{split}
    \Fstable_0''(t^{\epsilon}) &=
    \frac{
      \abs{z - \epsilon}^2\abs{z + \epsilon}^2e^{h^\epsilon}
      (\abs{z - \epsilon}^2e^{h^\epsilon} - \abs{z + \epsilon}^2)
    }{
      (\abs{z - \epsilon}^2e^{h^\epsilon} + \abs{z + \epsilon}^2)^3
    },\\
    \del_xv^{\epsilon} &=
    2\,
    \frac{
      (x - \epsilon)\abs{z + \epsilon}^2 - (x + \epsilon)\abs{z - \epsilon}^2
    }{
      \abs{z - \epsilon}^2\abs{z + \epsilon}^2
    }.
  \end{split}
\end{equation}

Recall the functions $h^\epsilon$ are uniformly bounded and use equation
\eqref{eq:uniform-conv-boundedness} to obtain, 

\begin{multline}
  \label{eq:5-ad}
  \abs*{\Fstable_0''(t^{\epsilon})}\left(\del_xv^{\epsilon}\right)^2 
  \leq
  \frac{
    4 C_2
  }{
    \left(
    \abs{z - \epsilon}^2 C_1 + \abs{z + \epsilon}^2
    \right)^2
  } \,
  \frac{
  \left(
    (x - \epsilon)\abs{z + \epsilon}^2 - (x + \epsilon)\abs{z - \epsilon}^2
  \right)^2 
}{
  \abs{z - \epsilon}^2 \abs{z + \epsilon}^2
}\\
\leq
\frac{
  4C_2(\abs{z - \epsilon}^2 + \abs{z + \epsilon}^2)
}{
  \left(
  \abs{z - \epsilon}^2C_2 + \abs{z + \epsilon}^2
  \right)^2
}.
\end{multline}

Comparing equation \eqref{eq:5-ad} with \eqref{eq:3-ad}, there is a constant
$C$ such that, 

\begin{equation}
  \label{eq:fdd-delxv-2-bound}
  \norm*{\Fstable_0''(t^{\epsilon})
    \left(\del_xv^{\epsilon}\right)^2}^2_{\Lsp^2(\sphere)} \leq
  \frac{C}{\epsilon^2}.
\end{equation}

Since $\Fstable_0''$ is a bounded function and the family $\dd h^\epsilon$ is
uniformly bounded,

\begin{align}
  \nonumber
  \norm*{
  \Fstable_0''(t^{\epsilon})\cdot\del_xv^{\epsilon}\cdot\del_x h^\epsilon
  }^2_{\Lsp^2(\sphere)} 
  &\leq   C_1 \norm*{
    \Fstable_0''(t^{\epsilon})(\del_xv^{\epsilon})^2
    }_{\Lsp^1(\sphere)}\\
  \nonumber
  &\leq
  C_2 \norm*{\Fstable_0''(t^{\epsilon})(\del_xv^{\epsilon})^2}_{\Lsp\sphere}\\
    \label{eq:fdd-delxvd-dexlhtilde-bound}
  &\leq \frac{
    C_3
    }{
    \epsilon
    }.
\end{align}

Combining equations
\eqref{eq:4-ad}, \eqref{eq:fdd-delxv-2-bound} and
\eqref{eq:fdd-delxvd-dexlhtilde-bound}, 
the boundedness of $\Fstable_0''$ and the fact that the family $h^\epsilon$ is bounded in $\Hsp^2(\sphere)$, there are constants $C_k$, $k =
1, \ldots, 5$, such that

\begin{equation}
  \label{eq:delx2-fstable}
  \norm*{\del_x^2\Fstable_0(t^{\epsilon})}_{\Lsp^2(\sphere)}
  \leq
  \frac{C_1}{\epsilon} + \frac{C_2}{\sqrt\epsilon} +
  C_3\norm*{\pbrk{\del_x h^\epsilon}^2}_{\Csp(\sphere)} +
  C_4\norm{h^\epsilon}_{\Hsp^2(\sphere)}
  \leq \frac{C_5}{\epsilon}.
\end{equation}

By \eqref{eq:laplace-plane-del2x-htildeeps-bound} and Sobolev's embedding,
there exists a constant $C$, such that,

\begin{equation}
  \label{eq:delx2-linf-bound}
  \norm*{\del_x^2 h^\epsilon}_{\Csp(\sphere)} \leq
  \frac{C}{\epsilon}. 
\end{equation}

\subsection{Uniform bounds for $\epsilon\del_\epsilon h^\epsilon$}
\label{sec:del-eps-htilde-eps-bound-2}

$\del_{\epsilon} h^\epsilon$ is a solution to the linear equation, 

\begin{equation}
  \label{eq:deleps-htilde-eps-equation}
  -\laplacian_{\sphere}\delEps h^\epsilon =
  \Fstable'(t^{\epsilon})(\delEps v^{\epsilon} + \delEps h^\epsilon).
\end{equation}

If we let
  $a = \Fstable'(t^\epsilon)$ and $b = \Fstable'(t^{\epsilon})\delEps
  v^{\epsilon}$, lemma~\ref{lem:linear-problem-bounds}  gives bounds for
  $\norm{\delEps h^\epsilon}_{\Hsp^2(\sphere)}$ in terms of  $\norm{a}_{\Lsp^2(\sphere)}$ and  $\norm{b}_{\Lsp^2(\sphere)}$. We note,

  \begin{equation}
    \label{eq:b-func}
    b = \frac{
      -32 x \abs{z}^2
    }{
      \left(
        \abs{z - \epsilon}^2\exp(h^\epsilon) +
        \abs{z + \epsilon}^2
      \right)^2
    }.
  \end{equation}

  After the change of variables $z \mapsto \epsilon w$, 

  \begin{align}
    \nonumber
    \norm{b}_{\Lsp^2(\sphere)}^2 &\leq \int_{\plane}\frac{
      C_1 \abs{w}^6
    }{\left(
     \abs{w - 1}^2C_2 + \abs{w + 1}^2
   \right)^4}
 \frac{
   d^2{w}
 }{
   \left( 1 + \epsilon^2\abs{w}^2 \right)^2
 }.\\
\nonumber
 &\leq
 \int_{\plane} \frac{
     C d^2{w}
   }{
     \left(
      1 + \epsilon^2\abs{w}^2
     \right)^2
   }\\
    \label{eq:b-l2-norm-bound}
   &= \frac{
     \pi C
   }{
     \epsilon^2
   }.
  \end{align}

 On the other hand, with the change of variables $z \mapsto \epsilon
 w^{-1}$, we arrive at 

 \begin{equation}
   \label{eq:a-fun-w-coords}
   \int_{\sphere}a \star 1 \geq \int_{\plane}
   \frac{
     C_1
     \abs{w - 1}^2\abs{w + 1}^2
   }{
     \left(
      \abs{w - 1}^2C_2 + \abs{w + 1}^2
     \right)^2
   } \frac{
     \epsilon^2d^2{w}
   }{
     \left(\epsilon^2 + \abs{w}^2\right)^2
   }.
 \end{equation}

The integral on the lower bound of \eqref{eq:a-fun-w-coords} is a
continuous positive function of $\epsilon$ for $0 < \epsilon \leq 1$,
because of the dominated convergence theorem. On the other hand, it
converges to the positive constant $C_1(1 + C_2)^{-2}$ as $\epsilon
\to 0$ by lemma~\ref{lem:mueps-delta-conv}. Therefore, there exists a
positive constant $C$ such that,

\begin{equation}
  \label{eq:integral-lower-bound}
  \int_{\sphere} a \star 1 \geq \frac{1}{C}.
\end{equation}

By lemma~\ref{lem:linear-problem-bounds}, there is another constant, also named $C$, such that

\begin{equation*}
    \norm{\delEps h^\epsilon}_{\Hsp^1(\sphere)} \leq \frac{C}{\epsilon},
\end{equation*}

Since $\delEps h^\epsilon$ is a solution of \eqref{eq:deleps-htilde-eps-equation}, by elliptic regularity,

\begin{equation}
\label{eq:del-eps-htilde-eps-bound-2}
    \norm{\delEps h^\epsilon}_{\Hsp^2(\sphere)} \leq 
    C_1 \norm{a}_{\Lsp^2({\sphere})}\,\norm{\delEps h^\epsilon}_{\Lsp^2({\sphere})} + \norm{b}_{\Lsp^2({\sphere})} \leq \frac{C_2}{\epsilon}.
\end{equation}

Therefore, Sobolev's embedding implies that the family $\epsilon\, \delEps h^\epsilon$ is uniformly bounded. 

\subsection{Uniform bound for $\epsilon\del_x\delEps h^\epsilon$}

Next, we estimate a bound for $\del_x\delEps h^\epsilon$. From
equation \eqref{eq:deleps-htilde-eps-equation},
$\del_x\delEps h^\epsilon$ is a solution to the equation,

\begin{equation}
  \label{eq:delx-u-elliptic-problem}
  -\laplacian_{\sphere}\del_x\delEps h^\epsilon =
  \frac{
    -4x\cdot(a\,\delEps h^\epsilon + b)
  }{
    (1 + \abs{z}^2)
  }
  + \del_x a\cdot\delEps h^\epsilon
  + a\,\del_x\delEps h^\epsilon
  + \del_x b.
\end{equation}

Let us define,

\begin{equation}
  \label{eq:bdash}
  b' =
  \frac{
    -4x\cdot(a\,\delEps h^\epsilon + b)
  }{
    (1 + \abs{z}^2)
  }
  + \del_x a\cdot\delEps h^\epsilon
  + \del_x b.
\end{equation}

A long calculation shows,

\begin{multline}
  \label{eq:delx-a}
  \del_x a = \frac{
    -16 e^{h^\epsilon} \abs{z - \epsilon}^2\abs{z + \epsilon}^2
  }{
    \left(\abs{z - \epsilon}^2e^{h^\epsilon} + \abs{z +
      \epsilon}^2\right)^3
  }\,
  \left(
    2(x - \epsilon)e^{h^\epsilon} + 2(x + \epsilon)
    + \abs{z - \epsilon}^2e^{h^\epsilon}\del_x h^\epsilon
  \right)\\
  +
  8\,
  \frac{
    2(x - \epsilon)\abs{z + \epsilon}^2e^{h^\epsilon}
    + 2\abs{z - \epsilon}^2(x + \epsilon)e^{h^\epsilon}
    + \abs{z - \epsilon}^2\abs{z + \epsilon}^2e^{h^\epsilon}\del_x h^\epsilon
  }{
    \left(
      \abs{z - \epsilon}^2e^{h^\epsilon} + \abs{z + \epsilon}^2
    \right)^2
  },
\end{multline}

and

\begin{multline}
  \label{eq:delx-b}
  \del_xb = \frac{
    -32(\abs{z}^2 + 2x^2)
  }{
    \left(
     \abs{z - \epsilon}^2e^{h^\epsilon} + \abs{z + \epsilon}^2
    \right)^2
  }\\
  +
  \frac{
    64 x\abs{z}^2 \left(
      2(x - \epsilon) e^{h^\epsilon}
      + \abs{z - \epsilon}^2 e^{h^\epsilon}
      \del_x h^\epsilon
      + 2(x + \epsilon)
    \right)
  }{
    \left(
     \abs{z - \epsilon}^2e^{h^\epsilon} + \abs{z + \epsilon}^2
    \right)^3
  }.
\end{multline}


From \eqref{eq:delx-a}, \eqref{eq:delx-b} and the change of variables $z \mapsto \epsilon w$, we infer the bounds

\begin{equation}
  \label{eq:delx-a-l2-bound}
  \norm{\del_xa}_{\Lsp^2(\sphere)} \leq \frac{C}{\epsilon}
\end{equation}

and 
\begin{equation}
  \label{eq:delxb-bound}
  \abs{\del_xb(\epsilon w)}_{\plane} \leq \frac{1}{\epsilon^2}
    \frac{
     \abs{w}^2 \sum_{k=0}^3 C_k\abs{w}^k
    }{
      \left(
        \abs{w - 1}^2 C_2 + \abs{w + 1}^2
      \right)^3
    },
\end{equation}

for some constants $C$, $C_k$, $k = 0, \ldots, 3$.
Therefore,

\begin{multline}
  \norm{\del_xb}_{\Lsp^2(\sphere)}^2 \leq \frac{
    1
  }{
    \epsilon^2
  }
  \int_{\abs{w}\geq 1} \frac{
    \abs{w}^{10}   \, d^2{w}
  }{
    \left(
        \abs{w - 1}^2 C_2 + \abs{w + 1}^2
      \right)^6
      \left(
        1 + \epsilon^2\abs{w}^2
      \right)^2
    }
    +
    \frac{
      1
    }{
      \epsilon^2
    }
    \int_{\abs{w} \leq 1}
    C d^2{w}.
\end{multline}

The second term in the bound is because the integrand is
a continuous function on a compact domain. For the first term, since
$\abs{\del_xb(\epsilon w)}$ is of order $\abs{w}^{-1}$
for big $\abs{w}$, there is another constant, still denoted $C$,
such that if we make the change of variables $w \mapsto w^{-1}$, then,

\begin{equation*}
  \int_{\abs{w} \geq 1} \frac{
    C d^2w
  }{
    \abs{w}^2 \left(
      1 + \epsilon^2\abs{w}^2
    \right)^2
  }
  =
  \int_{\abs{w} \leq 1}
  \frac{
    C \abs{w}^4d^2{w}
  }{
    \left(
      \abs{w}^2 + \epsilon^2
    \right)^2
  }
  \leq
  \pi C.
\end{equation*}

Hence,

\begin{equation}
  \label{eq:delx-bound}
  \norm{\del_xb}_{\Lsp^2(\sphere)} \leq \frac{
    C
  }{
    \epsilon
  }.
\end{equation}

From lemma~\ref{lem:linear-problem-bounds}, the estimate for $\delEps h^\epsilon$ found in section~\ref{sec:del-eps-htilde-eps-bound-2}, \eqref{eq:delx-a-l2-bound} and
\eqref{eq:delx-bound}, we conclude,

\begin{equation}
  \label{eq:bdash-bound}
  \norm{b'}_{\Lsp^2(\sphere)} \leq \frac{
    C
  }{
    \epsilon
  }.
\end{equation}

Therefore,

\begin{equation}
  \label{eq:h2-bound-delx-deleps-h}
  \norm{\del_x\del_{\epsilon} h^\epsilon}_{\Csp(\sphere)}
  \leq
  C_1 \norm{\del_x\del_{\epsilon} h^\epsilon}_{\Hsp^2(\sphere)} \leq \frac{
    C
  }{
    \epsilon
  }.
\end{equation}

Hence, $\epsilon \del_x \delEps h^\epsilon$ is also a famliy of uniformly bounded functions. 



\let \delEps \undefined
\let \cstar \undefined
\let \uniformlyto \undefined
\let \ctildeEps \undefined
\let \hstar \undefined
\let \htildeEps \undefined
\let \ctildeEps \undefined
\let \dd \undefined
\let \Csp \undefined





%%% Local Variables:
%%% TeX-master: "../../../geometric-models.tex"
%%% End:


==> chapters/vav-sphere/sections/linearised-problem-lemma.tex <==
\newcommand*{\aForm}{B}
\newcommand*{\ueps}{u}
\newcommand*{\hSp}{\mathcal{H}}
\newcommand*{\fFunc}{\mathcal{F}}
\newcommand*{\afn}{a}
\newcommand*{\bfn}{b}
\newcommand*{\manifold}{M}
\newcommand*{\metric}[1]{\langle #1 \rangle}





We will use Lax-Milgram's theorem to prove the following lemma.

\begin{lemma}
\label{lem:linear-problem-bounds}
Let $\manifold$ be any compact Riemannian manifold. If $\afn, \bfn \in
\Lsp^2(\manifold)$ such that $\afn$ is non-negative and bounded 
with positive integral $\int_\manifold \afn \star 1$. Then the linear problem,

\begin{equation}
  \label{eq:linear-problem}
  -\laplacian_{\manifold} \ueps = \afn\ueps + \bfn,
\end{equation}

has exactly one solution $u \in \Hsp^2(\manifold)$. Moreover, $u$
satisfies the bound, 

\begin{equation}
  \label{eq:u-bound}
  \norm{\ueps}_{\Hsp^2(\manifold)} \leq
  \frac{
    C
  }{
    \int_\manifold \afn \star1
  } \left(
    \frac{
      \norm{\afn}_{\Lsp^2(\manifold)}^2
    }{
      \int_\surface \afn \star1
    }
    + \norm{\afn}_{\Lsp^2(\manifold)}
    + 1
  \right)
  \norm{\bfn}_{\Lsp^2(\manifold)},
\end{equation}

for some positive constant $C$.
\end{lemma}
  

For comparison, see \cite{mitrea1999boundary,mitrea2000potential}
where a related problem is tackled.  

\begin{proof}
Let us define the space
%
\begin{equation*}
    \Xsp_\manifold = \left\{ \left.
    \tilde u \in \Hsp^1(\manifold) \right\rvert
    \int_\manifold u \star 1 = 0
    \right\},
\end{equation*}
%
of average zero functions in $\Hsp^1(\manifold)$. As for surfaces,
there is a natural splitting $\Hsp^1(\manifold) \cong \Xsp_\manifold
\times \reals$.  
Equation \eqref{eq:linear-problem} is equivalent to find 
$(\tilde\ueps_0, \tilde c) \in\Xsp_\manifold \times \reals$, such that 

\begin{equation}
  \label{eq:linear-prob-h10}
  -\laplacian_{\manifold} \tilde\ueps_0 = \afn\tilde\ueps_0 + \afn \tilde c + \bfn.
\end{equation}

By the divergence theorem, the constant is

\begin{equation}
  \label{eq:c-value}
  \tilde c = \frac{
   -\int_{\manifold} (\afn \tilde\ueps_0 + \bfn) \star 1
  }{
   \int_{\manifold}\afn\star 1
  }.
\end{equation}

Thence, (\ref{eq:linear-problem}) is equivalent to
find $\tilde\ueps_0 \in \Xsp$ such that

\begin{equation}
  \label{eq:h10-equiv-problem}
  -\laplacian_{\manifold} \tilde\ueps_0 = \afn \tilde\ueps_0 + \bfn - \frac{
    \afn \cdot \int_{\manifold} (\afn \tilde\ueps_0 + \bfn) \star 1
  }{
    \int_{\manifold}\afn \star 1
  }.
\end{equation}

Let us define the operators $\aForm:\Xsp_\manifold\times\Xsp_\manifold
\to \reals$, $\fFunc: 
\Xsp_\manifold \to \reals$, as

\begin{align}
\aForm(\tilde u, \tilde v) &= \int_\manifold \left(
    \metric{\dd \tilde \ueps, \dd \tilde v} + \afn \tilde\ueps \tilde v
  \right) \star 1
  - \frac{1}{\int_\manifold\afn \star 1}\,
   \int_\manifold \afn \tilde\ueps \star 1 \cdot\int_\manifold \afn \tilde v \star 1,\\
\fFunc(\tilde v) &=
\frac{
    1
  }{
    \int_\manifold\afn \star 1
  }
  \int_\manifold
  \left(
    \afn\cdot\int_\manifold\bfn \star1 - \bfn \cdot\int_\manifold\afn\star1
  \right)\cdot \tilde v \star1. 
\end{align}

% Equation (\ref{eq:h10-equiv-problem}) can be rewritten in variational form as the problem of finding $\tilde\ueps_0 \in\Xsp$, such that for any $\tilde v \in \Xsp$,

% \begin{equation}
%   \label{eq:variational-problem}
%   \aForm(\tilde\ueps_0, \tilde v) = \fFunc(\tilde v).
% \end{equation}

$\fFunc$ is bounded and $\aForm$ continuous because
$\afn, \bfn \in \Lsp^2(\manifold)$. By Cauchy-Schwartz inequality,

\begin{equation}
  \label{eq:cauchy-schwartz}
  \abs*{\int_\manifold \afn \tilde \ueps \star1} \leq
  \norm{\sqrt\afn}_{\Lsp^2(\manifold)}\norm{\sqrt\afn
    \tilde\ueps}_{\Lsp^2(\manifold)}, 
\end{equation}

hence,

\begin{equation}
  \label{eq:a-bil-coercive}
  \aForm(\tilde u, \tilde u) = \norm{\dd \tilde\ueps}_{\Lsp^2(\manifold)}^2
  + \frac{
    1
  }{
    \int_\manifold a \star1
  } \left(
    \int_\manifold a \tilde\ueps^2 \star1 \cdot \int_\surface a \star1
    -  \left(\int_\manifold a \tilde\ueps \star1\right)^2
    \right)
    \geq
    \norm{\dd\tilde\ueps}_{\Lsp^2(\manifold)}^2.
  \end{equation}


  By Poincar\'e's inequality, there is a positive
  constant $\alpha$, such that

  \begin{equation}
    \label{coercivity-A-H10}
    \alpha \norm{\tilde\ueps}_{\Hsp^1(\manifold)}^2 \leq \aForm(\tilde
    u, \tilde u).  
  \end{equation}

 Therefore, there exists a unique $\tilde u \in \Xsp_\manifold$
 satisfying~\eqref{eq:lax-milgram-problem}. For this function $\tilde
 u$, there exists only one constant  $\tilde c$ such that the function
 $u = \tilde u + \tilde c \in \Hsp^1(\manifold)$ is a weak solution of
 equation~\eqref{eq:linear-problem}. Since the right hand side of the
 equation is comprised of $\Lsp^2(\manifold)$ functions, $u \in
 \Hsp^2(\manifold)$. Moreover, by \eqref{eq:lax-milgram-bound}, this
 $\tilde u$ has the bound, 

\begin{equation}
  \label{eq:u0-F-bound}
  \norm{\tilde\ueps}_{\Hsp^2(\manifold)} \leq \frac{
    1
  }{
    \alpha\int_\manifold a \star1
  }\,\norm*{
    a\cdot\int_\manifold b\star1 - b\cdot\int_\manifold a \star1
  }_{\Lsp^2(\manifold)}. 
\end{equation}

By equation~(\ref{eq:c-value}),

\begin{equation}
  \label{eq:c-bound}
  \abs{\tilde c} \leq \frac{
    1
  }{
    \int_\manifold \afn \star1
  } \left(
    \norm{\afn}_{\Lsp^2(\manifold)}\cdot \norm{\tilde\ueps}_{\Lsp^2(\manifold)} +
    \abs*{\int_\manifold b \star1}
  \right).
\end{equation}

Therefore, $\ueps$ is bounded in $\Hsp^2(\manifold)$ by,

\begin{equation*}
  \norm{\ueps}_{\Hsp^2(\manifold)} \leq
  \frac{
    C
  }{
    \int_\manifold \afn \star1
  } \left(
    \frac{
      \norm{\afn}_{\Lsp^2(\manifold)}^2
    }{
      \int_\manifold \afn \star1
    }
    + \norm{\afn}_{\Lsp^2(\manifold)}
    + 1
  \right)
  \norm{\bfn}_{\Lsp^2(\manifold)},
\end{equation*}

for some suitable constant $C$.
\end{proof}


%  If we let $K$ be the bound for
% $\norm{\ueps}_{\Hsp\manifold}$ found in (\ref{eq:u-bound}), by the
% elliptic estimate for equation (\ref{eq:linear-problem}) and Sobolev's
% embedding theorem, we obtain the sequence of bounds,

% \begin{equation}
%   \label{eq:h2-bound-u}
%   \norm{\ueps}_{\Csp\manifold}
%   \leq
%   \norm{\ueps}_{\Hsp[2]\manifold} \leq \norm{\afn}_{\Lsp\manifold}\cdot
%   K + \norm{\bfn}_{\Lsp\manifold}.
% \end{equation}


\let \aForm \undefined
\let \ueps \undefined
\let \hSp \undefined
\let \fFunc \undefined
\let \afn \undefined
\let \bfn \undefined
\let \manifold \undefined
\let \metric \undefined





%%% Local Variables:
%%% TeX-master: "../../../geometric-models.tex"
%%% End:


==> chapters/vav-sphere/sections/param-dependency.tex <==

Since $\Fstable_0(v + h) \in \Lsp{\surface}$, we have that $h \in \Hsp[2]{\surface}$ by elliptic regularity, since in a closed manifold,

\begin{equation*}
\norm{h}_{\Hsp[2]{\surface}} \leq C \norm{\laplacian_\surface h}_{\Lsp{\surface}}.
\end{equation*}

Recall Sobolev's embedding \cite{aubin2013some} 

\begin{equation*}
\Hsp[2]{\surface} \to C^0(\surface),
\end{equation*}

hence $h$ is a continuous function. We will use the implicit function theorem in Banach spaces, as can be found in \cite[p.~72]{aubin2013some}.

\begin{theorem}[Implicit function theorem]
  Let $\mathfrak{E}, \mathfrak{F}, \mathfrak{B}$ be Banach spaces and
  $\mathfrak{U} \subset \mathfrak{E} \times \mathfrak{F}$ and open
  set. Suppose $f \in C^p(\mathfrak{U}, \mathfrak{B})$ and let
  $D_yf(x_0, y_0) \in \mathscr{L}(\mathfrak{F}, \mathfrak{B})$ be the
  differential at $y_0$ of the mapping $y \mapsto f(x_0, y)$. If at
  $(x_0, y_0) \in \mathfrak{U}$, $D_yf(x_0, y_0)$ is invertible, then
  the map $(x, y)\mapsto (x, f(x, y))$ is a $C^p$ diffeomorphism of a
  neighbourhood $\Omega \subset \mathfrak{U}$ of $(x_0, y_0)$ onto an
  open set of $\mathfrak{E} \times \mathfrak{B}$. 
\end{theorem}

By compactness, there is a minimal
injectivity radius $\rho$ such that for any $p \in \surface$, the
exponential map $\exp_p:T_p\surface \to \surface$ is a radial isometry at
least in the disk $\disk_{\rho}(p) \subset T_p\surface$.
For any $p
\in \surface$, there is an open neighbourhood $U$ of diameter lesser 
than $2 \rho$ such that if $r_p(x) = \dist(p,x)$, then

\begin{equation}
\label{eq:param-green-fnc-asymptotics}
G_p(x) = \frac{1}{4\pi}\log r_p(x)^2 + \tilde G_p(x),
\end{equation}
%
for some smooth remainder function $\tilde G_p \in C^{\infty}(U)$. In
this neighbourhood we also have that the squared distance function
$d(x, y)^2$ is a smooth function of both variables. In this neighbourhood, $v_p$ has the expansion 

\begin{equation}
\label{eq:vp-asympt-expansion}
v_p(x) = \log r_p(x)^2 + \tilde v_p(x),
\end{equation}

with $\tilde v_p$ a smooth function. If we consider a pair of points $(x, y) \in \surface\times\surface$
then we know that if $x \neq y$, the function $e^{v_x(y)}$ is
smooth. On the other hand, in a small neighbourhood $U$ of $x$ we
have,

\begin{equation}
\label{eq:exp-vx-asympt}
e^{v_x(y)} = r_x(y)^2e^{\tilde v_x(y)},
\end{equation}
%
since the distance function is smooth in this neighbourhood, we conclude that $e^{v_x(y)}$ is also smooth at points $(x, x)$ in the diagonal. Let
$\Delta\surface$ be the open subspace of  $\surface^{k_+}\times
\surface^{k_-}$ obtained removing all entries with repeated points. 
%then the function
%
%\begin{equation}
%\label{eq:vp-vq-x-fstab0}
%(\vp, \vq, x) \mapsto \Fstable_0\brk(v_\vp(x) - v_\vq(x))
%\end{equation}
%
%is smooth in $\Delta\surface \times \surface$. On the other hand,
Given a function $u \in \Hsp[r]\surface$, consider the exponential function
$e^u$. Pointwise,
%
\begin{equation}
\label{eq:exp-u-x}
e^{u(x)} = \sum_{n = 0}^{\infty}\frac{u(x)^n}{n!}.
\end{equation}

$\Hsp[r]\surface$ is a Banach algebra, given $u, v \in
\Hsp[r]\surface$, there is a constant $C(r) > 0$ such that

\begin{equation}
\label{eq:hsp-r-Banach-algebra}
\norm{uv}_{\Hsp[r]\surface} \leq C\,
\norm{u}_{\Hsp[r]\surface}\norm{v}_{\Hsp[r]\surface}.
\end{equation}

Hence $e^u \in \Hsp[r]\surface$, moreover, the operator $u \mapsto e^u$ is
smooth in $\Hsp[r]\surface$ because it is the limit of the absolutly
convergent series \eqref{eq:exp-u-x}. If we consider,

\begin{equation}
\label{eq:hr-fstable0}
\Fstable_0(u + v_{\vp} - v_{\vq}) = \frac{4
  e^u e^{v_{\vp}}}{e^ue^{v_{\vp}} + e^{v_{\vq}}} - C_0, 
\end{equation}
%
the functions $e^{v_{\vp}}$ and $e^{v_{\vq}}$ are smooth and without common
zeros and $e^u$ is a function positive almost everywhere, hence
$\Fstable_0(u + v_{\vp} - v_{\vq})$ is a well defined function 
$\Hsp[r]\surface \to \Hsp[r]{\surface}$.

Let $F:
\Delta\surface \times  \Hsp[r]{\surface} \to \Hsp[r - 2]{\surface}$  be the
functional,   

\begin{equation}
\label{eq:param-eq-functional}
F(\vp, \vq, u) = \laplacian_{\surface} u - \Fstable_0(u + v_\vp - v_\vq),
\end{equation}
%
if $(\vp, \vq, u) \in \Hsp[r]\surface$ is a solution to $F(\vp, \vq,
u) = 0$, by the  elliptic estimate,

\begin{equation}
  \label{eq:param-stnd-elliptic-estimate}
  \begin{aligned}[b]
    \norm{u}_{\Hsp[r + 1]\surface} &\leq C\,\brk( \norm{\laplacian
      u}_{\Hsp[r - 1]\surface} + \norm{u}_{\Hsp[r]\surface})\\
    &= C\,\brk( \norm{\Fstable_0(u + v_{\vp} - v_{\vq})}_{\Hsp[r -
  1]\surface} + \norm{u}_{\Hsp[r]\surface}) < \infty.
  \end{aligned}
\end{equation}

Given a configuration $(\vp, \vq)$, we know that there is a
solution $h \in \Hsp[2]\surface$ of the governing elliptic problem, by equation 
\eqref{eq:param-stnd-elliptic-estimate} $h \in
\Hsp[r]\surface$ for all $r \in \mathbb{N}$. By Sobolev's embedding, 

\begin{equation}
\label{eq:param-sob-embedding}
\norm{h}_{C^{r - 2}(\surface)} \leq C(r)\,\norm{h}_{\Hsp[r]\surface} <
\infty,
\qquad r \geq 2.
\end{equation}

Therefore, a solution of \eqref{eq:regular-taubes-bps} is smooth. We
aim to apply the implicit function theorem to prove that the
solution $h(x; \vp, \vq)$ depends smoothly on the input data $(\vp,
\vq)$. We work in local coordinates in $\Delta\surface$, hence, assume
we have chosen non-intersecting coordinate 
neighbourhoods $U$ for each $p$ or $q$ in which the metric $g$ is
conformally flat, 

\begin{equation}
\label{eq:param-conf-condition}
g = g_{12}\,(dx_1^2 + dx_2^2), \qquad x \in U.
\end{equation}

Let $\Delta U$ be the cartesian product of such neighbourhoods in
$\Delta\surface$. Up to diffeomorphism, we can suppose $\Delta U =
\reals^{k_+}\times \reals^{k_-}$ with the pullback metric. Let
%
\begin{equation}
\label{eq:param-domain-def}
\domain = \reals^{k_+}\times \reals^{k_-} \times \Hsp[k]\surface,
\end{equation}
%
we will prove that $F$ is a smooth operator in $\domain$. To see this, consider that
$e^{v_{\vp}}$ and $e^{v_{\vq}}$ are smooth functions defined in
$\reals^{k_+}\times\surface \to \reals$ and
$\reals^{k_-}\times\surface \to \reals$ 
respectively and the operator $u \mapsto e^u$ is smooth as a
functional $\Hsp[r]\surface \to \Hsp[r]\surface$. If we let $f$ be the smooth function

\begin{equation}
\label{eq:param-smooth-real-func}
f(a, b, c) = \frac{4 ac}{ac + b} - C_0,
\end{equation}

defined in the open subset of $\reals^3$ such that $ac + b \neq 0$, then
$\Fstable_0 = f \brk(e^{v_{\vp}}, e^{v_{\vq}}, u)$ is again a
smooth function. Let us consider now the derivative $\Diff_uF \in
\mathscr{L}\brk(\Hsp[r]\surface, \Hsp[r - 2]\surface)$ at a zero
$(\vp, \vq, h)$ of $F$, 

\begin{equation}
  \label{eq:param-delu-F}
  \begin{aligned}[b]
    \Diff_uF(\vp, \vq, h)\, \delta u
    &= \laplacian_{\surface} \delta u - \Fstable_0'\brk(h + v_{\vp} -
    v_{\vq})\,\delta u \\
    &=\laplacian_{\surface} \delta u - \frac{4
  e^{v_{\vq}} e^{v_{\vp}} e^h}{
  \brk( e^h e^{v_{\vp}} + e^{v_{\vq}})^2}\,\delta u,
  \end{aligned}
\end{equation}

We will denote  $\Fstable_0'\brk(h + v_{\vp} - v_{\vq})$
as $\Fstable_0'$. If $\delta u \in \operatorname{Ker} \Diff_uF$,

\begin{equation}
  \label{eq:param-ker-condition}
  \begin{aligned}
    0 &= \lproduct{\delta u, \laplacian_{\surface} \delta u}_{\Lsp\surface} -
    \lproduct{\delta u, \Fstable_0'\,\delta u}_{\Lsp\surface}\\
    &= - \norm{d\delta u}_{\Lsp\surface} -
    \norm*{\sqrt{\Fstable_0'}\,\delta u}_{\Lsp\surface} \leq 0.
  \end{aligned}
\end{equation}

Hence, $\delta u = 0$ almost everywhere and $\Diff_uF$ is
injective. Since $\Fstable_0'\in \Lsp\surface$ is positive and
bounded, as shown in lemma~\ref{lem:linear-problem-bounds} of section~\ref{sec:elliptic-sphere}, for any $w \in
\Hsp[r - 2]\surface$, there is $\delta u \in \Hsp[1]\surface$ such that,

\begin{equation}
\label{eq:param-h1-sol-linear-problem}
\laplacian_{\surface}\,\delta u - \Fstable_0'\,\delta u = w.
\end{equation}

Notice that $\Fstable_0' \in \Hsp[r]\surface$ and since $\Hsp[k]\surface$
is an algebra for any $k \geq 0$, by the standard elliptic estimates,
we infer from \eqref{eq:param-h1-sol-linear-problem} that $\delta u
\in \Hsp[r]\surface$. Therefore, $\Diff_uF$ is bijective and by the
open mapping theorem, it is an isomorphism of Banach spaces. We
conclude from the implicit function theorem that the family of
solutions $h(x; v_{\vp}, v_{\vq}) \in C^{\infty}(\surface)$ varies
smoothly as functions $\surface^{k_+} \times \surface^{k_-} \to \Hsp[r]\surface$
for any $r \geq 0$. Hence, solutions,

\begin{equation}
\nonumber
u = h + v_{\vp} - v_{\vq},
\end{equation}
%
to the governing elliptic problem have the regularity claimed in
theorem~\ref{thm:main}. 


%%% Local Variables:
%%% mode:
%%% TeX-master: ../../../geometric-models.tex
%%% End:



==> chapters/vav-sphere/sections/proof-incompleteness.tex <==
\newcommand*{\length}{\ell}

We aim to show that moduli space $\moduli^{1,1}(\sphere)$ is incomplete by showing
the geodesic trajectory $\epsilon \mapsto q(\epsilon)$, $\epsilon \in (0,1]$ is of
finite length, yet $q(0)$ is not in moduli space. The length of this path is, 
% The energy of this
% path is 

% \begin{equation}
%   \label{eq:energy-path}
%   E = \frac{1}{2} \int_0^1 g(-E_0, -E_0)\, d\epsilon, 
% \end{equation}
%
\begin{align}
  \length &= \int_0^1 g(-E_0, -E_0)^{1/2}\, d\epsilon 
  \nonumber\\
  &=\sqrt{2\pi}\int_0^1
  \left(
    \frac{8R^2}{(1 +\epsilon^2)^2} + \frac{1}{\epsilon} \dv\epsilon
    (\epsilon\cdot b_1)
  \right)^{1/2}d\epsilon,
  \label{eq:length-path}
\end{align}
%
and is bounded by,

\begin{equation}
  \label{eq:length-bound}
  \length \leq \pi\sqrt{\pi}R + \sqrt{2\pi} \int_0^1 \left(
  \frac{1}{\epsilon} \dv\epsilon (\epsilon\cdot b_1)
  \right)^{1/2}d\epsilon.
\end{equation}

On the other hand,

\begin{equation}
  \label{eq:diff-eps-b1}
  \dv\epsilon (\epsilon\cdot b_1) = 2 \dv\epsilon
  (\epsilon\del_x h^\epsilon(\epsilon)) = 2\left(
  \del_x h^\epsilon(\epsilon) +
  \epsilon\eval{\del_{\epsilon}\del_x h^\epsilon}{z=\epsilon} +
  \epsilon\del^2_x h^\epsilon(\epsilon)
  \right).
\end{equation}

We know from the estimates \eqref{eq:delx2-linf-bound}, \eqref{eq:del-eps-htilde-eps-bound-2}
 and \eqref{eq:h2-bound-delx-deleps-h} that
this derivative is uniformly bounded, thence, there is a
constant $C$, such that,

\begin{equation}
  \label{eq:ell-bound}
  \ell \leq \pi\sqrt\pi R + \sqrt{2\pi} C
  \int_0^1\epsilon^{-1/2}d\epsilon
  = \sqrt\pi \left(
    \pi R + 2\sqrt 2 C
    \right).
\end{equation}

This shows there is a maximal geodesic of finite length. Therefore,
moduli space is geodesically incomplete.


\let \length \undefined


==> chapters/vav-sphere/sections/uniqueness.tex <==
This follows from the maximum principle and the monotonicity of the function $\Fstable_0$.


==> leeds-style/Abbreviations/Abbreviations.tex <==
\newcommand*\Diff{\mathrm{D}}
\newcommand*{\confSp}{\mathcal{C}}
\newcommand*{\gaugeGp}{\mathcal{G}}
\newcommand*{\fieldSp}{\fieldConfSpace}
\newcommand*{\cDiff}{\mathcal{D}}
\newcommand*{\vset}{\mathcal{P}}
\newcommand*{\avset}{\mathcal{Q}}
\newcommand*{\Wsp}{\mathrm{W}}
\newcommand*{\Hsp}{\mathrm{H}}
\newcommand*{\kmetric}{\mathrm{K}}
\newcommand*{\connSp}{\connectionSpace}


\begin{abbreviations}

%Place your abbreviations in here...

\begin{table}[h]
\centering
\begin{tabular}{ll}
$\mathbb{P}^1$  & Complex projective space \\
$\surface$ & Riemann's surface \\
  $\gaugeGp$ & Gauge group \\
  $\connSp$  & Space of connections\\
  $\fieldSp$ & Space of fields \\
  $\fieldSp'$ & Space of solutions to Bogomolny's equations\\
  $\confSp$   & Configuration space\\
  %$\Diff$     & Covariant derivative on moduli space\\
  $\nabla$    & Covariant derivative of tensors on $\surface$\\
  $\laplacian$ & Geometer's Laplacian\\
  $\vset$     & Set of vortices\\
  $\avset$    & Set of antivortices\\
  $\moduli^{k_+,k_-}(\surface)$ & Moduli space of $k_+$ vortices and
                                  $k_-$ antivortices\\
  $\moduli^{k_+,k_-}_0$ & Reduced moduli space on the plane\\
  $\kmetric$   & K\"ahler's metric on moduli space\\
  $\Wsp^{k,p}$  & Generic Sobolev's space \\
  $\Hsp^k$     & Sobolev's space with $p = 2$\\
  $\norm{\cdot}_k$ & Norm on $\Hsp^k$\\
  $\norm{\cdot}_{k,p}$ & Norm on $\Wsp^{k,p}$\\
\end{tabular} 
\label{tbl:Abbreviations}
\end{table}


\end{abbreviations}


\let\connSp \undefined 
\let\kmetric \undefined
\let\Hsp \undefined 
\let\Wsp \undefined 
\let\Diff \undefined 
\let\confSp \undefined 
\let\gaugeGp \undefined 
\let\fieldSp \undefined 
\let\confSp \undefined 
\let\cDiff \undefined 
\let\vset \undefined 
\let\avset \undefined 


==> leeds-style/Acknowledgement/acknowledgement.tex <==
% Thesis Acknowledgements ------------------------------------------------


%\begin{acknowledgementslong} %uncommenting this line, gives a different acknowledgements heading
\begin{acknowledgements}      %this creates the heading for the acknowlegments

I would like to thank my supervisor, Martin Speight, for his valuable guidance 
and support. His experience and insight were encouraging and motivating, which 
I truly appreciate.

My gratitude to Derek Harland and Bernd Schroers for their comments on the 
final version of this thesis. 

Many thanks to my family and friends for their kind support both 
at Leeds and abroad through 
constant calls and messages, specially to Eyra for her support at 
home and to Diana who shared with me so many moments even at the distance.

This project would have not been possible without the support of 
CONACyT through a PhD grant which I kindly acknowledge.




\end{acknowledgements}
%\end{acknowledgmentslong}

% ------------------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> leeds-style/Dedication/dedication.tex <==
% Thesis Dedictation ---------------------------------------------------

\begin{dedication} %this creates the heading for the dedication page

To my daughter.

\end{dedication}

% ----------------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 

